Shape-Aware Fine-Grained Classification of Erythroid Cells

Fine-grained classification and counting of bone marrow erythroid cells are vital for evaluating the health status and formulating therapeutic schedules for leukemia or hematopathy. Due to the subtle visual differences between different types of erythroid cells, it is challenging to apply existing image-based deep learning models for fine-grained erythroid cell classification. Moreover, there is no large open-source datasets on erythroid cells to support the model training. In this paper, we introduce BMEC (Bone Morrow Erythroid Cells), the first large fine-grained image dataset of erythroid cells, to facilitate more deep learning research on erythroid cells. BMEC contains 5,666 images of individual erythroid cells, each of which is extracted from the bone marrow erythroid cell smears and professionally annotated to one of the four types of erythroid cells. To distinguish the erythroid cells, one key indicator is the cell shape which is closely related to the cell growth and maturation. Therefore, we design a novel shape-aware image classification network for fine-grained erythroid cell classification. The shape feature is extracted from the shape mask image and aggregated to the raw image feature with a shape attention module. With the shape-attended image feature, our network achieved superior classification performance (81.12\% top-1 accuracy) on the BMEC dataset comparing to the baseline methods. Ablation studies also demonstrate the effectiveness of incorporating the shape information for the fine-grained cell classification. To further verify the generalizability of our method, we tested our network on two additional public white blood cells (WBC) datasets and the results show our shape-aware method can generally outperform recent state-of-the-art works on classifying the WBC. The code and BMEC dataset can be found on https://github.com/wangye8899/BMEC.

==> 00abstraction.tex <==
\abstract{
Fine-grained classification and counting of bone marrow erythroid cells are vital for evaluating the health status and formulating therapeutic schedules for leukemia or hematopathy.
Due to the subtle visual differences between different types of erythroid cells, it is challenging to apply existing image-based deep learning models for fine-grained erythroid cell classification. 
Moreover, there is no large open-source datasets on erythroid cells to support the model training.
In this paper, we introduce BMEC (Bone Morrow Erythroid Cells), the first large fine-grained image dataset of erythroid cells, to facilitate more deep learning research on erythroid cells.
BMEC contains 5,666 images of individual erythroid cells, each of which is extracted from the bone marrow erythroid cell smears and professionally annotated to one of the four types of erythroid cells.
To distinguish the erythroid cells, one key indicator is the cell \textit{shape} which is closely related to the cell growth and maturation.
Therefore, we design a novel shape-aware image classification network for fine-grained erythroid cell classification. 
The shape feature is extracted from the shape mask image and aggregated to the raw image feature with a shape attention module.
With the shape-attended image feature, our network achieved superior classification performance (81.12\% top-1 accuracy) on the BMEC dataset comparing to the baseline methods. 
To further verify the effectiveness of our method, we tested our network on two additional public white blood cells (WBC) datasets.
The results show our shape-aware method can generally outperform recent state-of-the-art work on classifying the WBC.
The code and BMEC dataset can be found on \url{https://github.com/wangye8899/BMEC}.
}

==> 01introduction.tex <==
\section{Introduction}
The erythrocytes or red blood cells are one of the most critical cells in the body. There are four types of erythroid cells (Figure \ref{fig:cell_type}) based on their growth and maturation.
%: proerythroblast, basophilic erythroblast, polychromatophilic erythroblast, and orthochromic erythroblast.
In a healthy body, they maintain a relatively balanced state. However, in many blood disorders such as anemia, the number of these erythroid cells will change and become unbalanced. 
Therefore, the \textit{fine-grained} classification and counting of different types of erythroid cells are vital in diagnosing and preventing the related diseases \cite{chitra2019detection}.

\rui{One typical way} for cell classification and counting is to manually observe the morphological or shape differences of the cells through the microscope. 
Such process relies heavily on the hematologists' experience and skills, and it is easy to make mistakes and introduce subjectivity to the results.
Furthermore, it may take several years to train a competent hematologist to distinguish the specific type of erythroid cells.
In recent years, several image processing and machine learning techniques for classifying and counting erythroid cells have been proposed.
Most existing methods \cite{alomari2014automatic,lippeveld2020classification,petrovic2020sickle} mainly \rui{follow the traditional machine learning pipeline}, including data prep-processing, feature extraction, feature selection, and classification steps.
%Even though these techniques have demonstrated exemplary performance, their pre-processing is redundant and has poor robustness and generalization to other data. In addition, these techniques do not fully exploit and utilize the morphological differences between erythroid cells.
% \rui{Even though satisfied performance has been achieved, these methods rely on manually designed features which may constrain the generalizability of the classification model.
% In addition, the morphological and shape differences are not fully and deeply exploited in the model.}
% \ruim{[Rui: did these methods do fine-grained classification?]}
% \wy{[Reply: No work focus on the fine-grained classification for Erythroid cells. Most of these works research the WBCs' fine-grained classification.]}
Since these methods rely on manually designed features, the generalizability of the classification model may be limited.
In addition, the morphological and shape differences are not fully and deeply exploited in the model.
Even though satisfied results have been achieved for classifying white blood cells or certain abnormal types of erythroid cells whose shapes are visibly distinctive, traditional methods may not perform well for fine-grained classification of erythroid cells with only subtle shape differences. 


On the other hand, deep learning techniques have shown superior performance than traditional machine learning methods in computer vision tasks such as image classification \cite{liu2021swin}, object detection \cite{xu2021end} and segmentation \cite{strudel2021}.
%and their powerful feature representation and learning capabilities have overcome the shortcomings of the above methods. 
Deep neural networks can automatically extract deep image features which are more robust and more generalizable than hand-crafted features. 
However, most pre-trained network models \cite{simonyan2014very, he2016deep, huang2017densely, HangZhang2020ResNeStSN, liu2021swin} cannot directly learn the subtle shape differences which are crucial for fine-grained classification of erythroid cells.
To enable fine-grained erythroid cell classification, a more customized and shape-aware network needs to be designed and trained on erythroid cell images with finer-level category annotation.
%In addition to the technical difficulties mentioned above, the scarcity of open-source erythroid cell datasets poses another challenge for erythroid cells study.
Unfortunately, unlike the leukocytes or white blood cells (WBC), for which many open-source datasets are available (e.g., LISC \cite{rezatofighi2011automatic}, BCCD \cite{mohamed2012efficient} and Raabin-WBC \cite{kouzehkanan2021raabin}), \rui{there is no existing open-source fine-grained datasets to support the deep learning on erythroid cells}.

%Although the deep network can be trained on the WBCs datasets and fine-tuned on some erythroid cell images via transfer learning techniques, 
%Many leukocyte datasets have been open-sourced, such as Raabin-WBC\cite{kouzehkanan2021raabin}, LISC\cite{rezatofighi2011automatic}, and BCCD\cite{mohamed2012efficient} datasets. With this comes an increasing number of studies on leukocyte classification.
%However, due to the lack of open-source datasets for erythroid cells, relatively few works have been done. 
%Another reason for the low number of relevant research is that erythroid cells' morphological differences are too subtle compared to leukocytes. It is incredibly challenging to classify and count erythroid cells.

In this paper, we introduce BMEC (Bone Morrow Erythroid Cells), a large fine-grained image dataset of erythroid cells, to facilitate the study for erythroid cells in real clinical scenarios.
BMEC dataset contains 5,666 images of individual erythroid cells.
Each image contains one erythroid cell extracted from the bone marrow erythroid cell smears and is annotated to one of the four types of erythroid cells by the hematologists (Figure \ref{fig:cell_type}).
To classify the erythroid cells into fine-grained categories, we propose a novel \textit{shape-aware} image classification model which explicitly encode the shape information into the network (Figure \ref{fig:overview}).
Specifically, we first extract the cell shape mask image from the input erythroid cell image.
Then, the shape mask feature and the input image feature are extracted using the existing backbone image feature extraction models.
A shape attention module is further employed to compute a shape-attended image feature, which is aggregated to the shape feature and the raw image feature to form a fused feature for final classification.
% Furthermore, this paper attempts to explore how the shape information of erythroid cells can be used to improve the classification. 
% To efficiently classify a large volume of images, we develop a novel classification method based on shape attention and Swin-Transformer\cite{liu2021swin}. 
 
We conducted extensive quantitative evaluations of different backbone models for our shape-aware network on BMEC and our final model with Swin-Transformer \cite{liu2021swin} and VGG19 \cite{simonyan2014very} achieved 81.12\% top-1 accuracy which is consistently superior than other backbone model combinations.
We also performed ablation studies to verify the effectiveness of explicitly using shape information for fine-grained erythroid cell classification.
Furthermore, we tested our shape-aware classification network on two public leukocytes or WBC datasets and the results show our method can outperform recent state-of-the-art work on classifying the WBC.
%The results show that our method not only make full use of erythrocyte shape information to facilitate classification but also surpasses the accuracy of recent state-of-the-art leukocyte classification methods on the three leukocyte datasets.
In summary, our contributions are as follows:

\begin{itemize}
\item We introduce BMEC, the first large dataset of erythroid cell images with fine-grained category annotation, to support more deep learning research on erythroid cells. This dataset contains 5,666 professionally annotated images of four types of erythroid cells, while there are only subtle shape differences between these fine-grained types, making our dataset more chanllenging than existing WBC datasets.


%\item We design a simple but effective shape attention module inspired by \textcolor{wy}{cross attention\cite{SatyamMohla2020FusAtNetDA} for highlighting and fusing cell shape information to improve classification accuracy. To our knowledge, we are the first to utilize the attention mechanism to extract cell shape features for improving the fine-grained erythroid cell classification.}

\item We design a novel shape-aware network which employs a shape attention module to compute a shape-attended image feature and uses the shape-aggregated feature to improve the fine-grained classification accuracy of erythroid cells.
To our best knowledge, we are the first to explicitly incorporate the shape information to the deep learning framework for this task.

% \item We develop a novel fine-grained erythroid cell classification scheme based on the Swin-Transformer\cite{liu2021swin} and combined it with the shape attention module. 
% Experimental results on BMEC dataset introduced by us  and three public WBCs datasets demonstrate the effectiveness of our approach.

\item We perform extensive evaluations of our network with different backbone models and conduct ablation studies to verify the effectiveness of shape information.
The results on BMEC and two other WBC datasets show the superiority of the proposed shape-aware network and models in classifying the blood cell images.
\end{itemize} 

==> 02related_work.tex <==
\section{Related Work}


% \begin{table*}[h!t]
% \centering
% \small
% %\resizebox{\columnwidth}{!}{
% \begin{tabular}{c c c c c c}
% \toprule
% Dataset    & Number of images & Cell type       & Number of categories & Label         & Microscope                            \\ \hline
% LISC \cite{rezatofighi2011automatic}      & 266              & WBC             & 5                    & one expert    & Axioskope40                           \\ 
% BCCD \cite{mohamed2012efficient}       & 349              & WBC             & 5                    & one expert    & Regular light microscope              \\ 
% MISP       & 149              & WBC             & 4                    & one expert    & Canon optical microscope              \\ 
% ALL-IDB    & 84               & WBC             & 5                    & one expert    & N/A                                   \\ 
% Raabin-WBC \cite{kouzehkanan2021raabin} & 17,965            & WBC             & 5                    & two experts   & Olympus Cx18 \\ 
% BMEC       & 5,666             & Erythroid cells & 4                    & three experts & Olympus BX43                                   \\ 
% \bottomrule
% \end{tabular}
% %}
% \caption{Comparing other datasets with BMEC dataset. \ruim{[Rui: MISP and ALL-IDB are not mentioned and compared. Delete them? Add CBC and erythrocytesIDB? The image numbers are not the same as in Sec 2.1, double check. Change the table styles like this one for all other tables.]}}
% \label{tab:datasets}
% \end{table*}

% \begin{table}[h]
% \begin{center}
% \begin{minipage}{174pt}
% \caption{Caption text}\label{tab1}%
% \scalebox{0.6}{

% \begin{tabular}{@{}llllll@{}}
% \toprule
% Dataset& Quantity& Cell Type& Classes& Label& Microscope\\
% \midrule
% LISC \cite{rezatofighi2011automatic}& 250& WBC& 5& one expert& Axioskope40\\  
% BCCD \cite{mohamed2012efficient}    & 349& WBC& 5& one expert    & Regular light microscope\\
% Raabin-WBC\cite{kouzehkanan2021raabin}& 17,965& WBC& 5& two experts& Olympus Cx18\\     
% CBC \cite{alam2019machine} & 360& Erythroid cells& 3& two experts& ECLIPSE 50i microscope\\
% erythrocytesIDB \cite{gonzalez2014red} & 629& Erythroid cells & 3& one expert& Leika microscope\\
% BMEC (ours) & 5,666& Erythroid cells & 4& three experts & Olympus BX43 \\
% \botrule
% \end{tabular}
% }

% \end{minipage}
% \end{center}
% \end{table}

\begin{table}[h]

\begin{center}
\begin{minipage}{350pt}
\caption{Comparison of related WBC and erythroid cell datasets with our BMEC.}\label{tab:datasets}%
\centering
\begin{tabular}{@{}llllll@{}}
\toprule
Dataset& Quantity& Cell Type& Classes& Label& Microscope\\
\midrule
LISC \cite{rezatofighi2011automatic}& 250& WBC& 5& one expert& Axioskope40\\  
BCCD \cite{mohamed2012efficient}    & 349& WBC& 5& one expert    & Regular light micro\\
Raabin-WBC\cite{kouzehkanan2021raabin}& 17,965& WBC& 5& two experts& Olympus Cx18\\     
CBC \cite{alam2019machine} & 360& Erythroid cells& 3& two experts& ECLIPSE 50i micro\\
erythrocytesIDB \cite{gonzalez2014red} & 629& Erythroid cells & 3& one expert& Leika micro\\
BMEC (ours) & 5,666& Erythroid cells & 4& three experts & Olympus BX43 \\
\botrule
\end{tabular}
\end{minipage}
\end{center}
\end{table}


% \begin{table*}[h!t]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% Dataset      & Quantity & Cell Type       & No. of Categories & Label         & Microscope               \\ \hline
% LISC \cite{rezatofighi2011automatic}         & 250              & WBC             & 5                    & one expert    & Axioskope40              \\ \hline
% BCCD \cite{mohamed2012efficient}         & 349              & WBC             & 5                    & one expert    & Regular light microscope \\ \hline
% Raabin-WBC \cite{kouzehkanan2021raabin}   & 17,965           & WBC             & 5                    & two experts   & Olympus Cx18             \\ \hline
% CBC \cite{alam2019machine}          & 360              & Erythroid cells          & 3                    & two experts   & ECLIPSE 50i microscope   \\ \hline
% erythrocytesIDB \cite{gonzalez2014red} & 629              & Erythroid cells & 3                    & one expert    & Leika microscope         \\ \hline
% BMEC (ours)         & 5,666            & Erythroid cells & 4                    & three experts & Olympus BX43             \\ \hline
% \end{tabular}
% \caption{Comparison of related WBC and erythroid cell datasets with our BMEC.
% }
% \label{tab:datasets}
% \end{table*}

In this section, we first discuss several datasets on blood cells, including both leukocytes and erythrocytes, with the emphasis on the data characteristics and how they are collected; see Table \ref{tab:datasets}. 
We then provide a brief review of the traditional and deep learning techniques related to blood cell classification and counting.

\subsection{Blood Cell Datasets}
\textbf{WBC datasets.} There are many available white blood cell image datasets for investigating the WBC classification and counting tasks \cite{rezatofighi2011automatic,mohamed2012efficient,labati2011all,zheng2018fast,naruenatthanaset2020red,kouzehkanan2021raabin}.
% We then describe the characteristics of each dataset in detail.
Here, we only describe three representative WBC datasets and highlight their difference with our BMEC; see Table \ref{tab:datasets}.
The LISC \cite{rezatofighi2011automatic} is an early WBC dataset that includes the hematological images taken from peripheral blood of healthy subjects.
The smears were stained by through the Gismo-right technique and a Sony Model No.SSCDC50AP camera was used to capture the observation of a Axioskope 40 microscope at 100X magnification. 
Then, 250 WBC images were extracted and labelled by one blood expert into five fine-grained categories.
% It contains 257 WBCs images which only one blood expert has labeled. LISC dataset has been stained through the Gismo-right technique, and all images have been taken at a magnification of 100 using Microscope-Axioskope 40 microscope and a Sony Model No.SSCDC50AP camera.
%LISC dataset has been stained through the Gismo-right technique, and all images have been taken at a magnification of 100 using Microscope-Axioskope 40 microscope and a Sony Model No.SSCDC50AP camera.
%
Similarly, BCCD \cite{mohamed2012efficient} contains 349 WBC images that have been taken from peripheral blood and annotated by one expert.
The smears were also stained by the Gismo-right technique and the observations of a regular light microscope at 100X were captured using a CCD color camera.
Each WBC image extracted from the smear image was annotated by one expert into one of five categories.
Raabin-WBC \cite{kouzehkanan2021raabin} is a recent, large and public dataset of white blood cell images extracted from the normal peripheral blood samples. 
The peripheral blood smears were stained by the Giemsa technique and the images were taken using a Samsung Galaxy S5 camera \rui{to capture the observation of an Olympus CX18 microscope at 100X magnification}. 
% In addition, CML (Chronic Myeloid
% Leukemia) slices were imaged using an LG G3 camera phone and a Zeiss brand microscope. 
%Notably, these images were taken at a magnification of 100.
%It contains a total of 40,000 cropped images of WBCs and artifacts (color spots) for classification.
% This dataset has three subsets, Train, Test-A, and Test-B, respectively. 
% In total, 17,965 cropped images, each of which contain \rui{a central WBC} and other artifacts (color spots) are provided.
\wy{In total, 17,965 WBCs images are cropped from the smear images and labelled into five categories by two blood experts. }
% The cropped images were labelled by two blood experts into five categories for classification.
% \ruim{[Rui: how the WBC image were cropped from the smear image, by expert?]}
% % Table \ref{tab:datasets}
% \wy{[Reply: Yes, the two experts have cropped these images with the help of android and desktop applications. However, our dataset are cropped  manually by three experts. I think that this is not our strength compared to Raabin-WBC. Therefore, I did not introduce the cropping process in detail.]}
Comparing to the white blood cells, different types of erythroid cells look more similar and the shape difference between the types is subtle.
Therefore, it is more challenging for fine-grained erythroid cell classification, e.g., over 99\% accuracy can be achieved on Raabin-WBC while only around 80\% accuracy can be obtained on our BMEC.
Due to the difficulty on distinguishing the erythroid cell types, we asked three hematologists to jointly label the BMEC images in a more rigorous manner.

\textbf{Erythroid cell datasets.} Compared to the WBC datasets, there are only a few  open-source datasets containing the erythrocytes, while the data quality, quantity and variety are limited comparing to our BMEC.
As shown in Table \ref{tab:datasets}, CBC \cite{alam2019machine} is a hybrid dataset which contains three types of blood cells: red blood cells, white blood cells, and platelets.
\wy{The images in CBC were taken using a Nikon V1 camera to capture the observation of an ECLIPSE 50i microscope at 100X magnification, and then annotated by two experts.}
% \wy{[Reply: The related details and content have been added.]}
It focuses more on investigating the differences between the three types of blood cells rather than classifying red blood cells into fine-grained types. In addition, CBC only has 360 images which are difficult for training the deep neural networks.
One most related dataset on erythroid cell classificaiton is the erythrocytesIDB \cite{gonzalez2014red} which contains 629 images of individual erythroid cells extracted from 196 full filed peripheral blood images. 
A Kodak EasyShare V803 camera was used to capture the observation of a Leika microscope at 100X magnification.
%Even though it further divides the erythroid cells into three categories, the number of images is still low.
The erythrocytesIDB images are annotated by \wy{one} expert into three categories based on the cell shape: circular, elongated and other shape.
Comparing to BMEC, the shape differences for erythroid cells in erythrocytesIDB are more significant since they focus on the study in cell deformation caused by certain blood diseases.
Hence, it's much easier to achieve high accuracy (98\% in \cite{gonzalez2014red}) on erythrocytesIDB.
In contrast, our BMEC provides a much larger number of images with minor shape differences, so that it can be used to train a more generalizable deep learning model for fine-grained erythroid cell classificaiton.

%In summary, there is an urgent need for an erythroid cell dataset with an abundant amount of data and a wide variety of cells.


\subsection{Cell Classification Techniques}
% \subsection{Descripción del Diseño del experimento }
% \subsection{Toma de datos}
% \subsection{Análisis de información y recursos utilizados}
% As more and more blood cell datasets are open-sourced, excellent methods and researches on blood cells classification have been proposed. 
% These techniques can be divided into image processing, machine learning techniques, and deep learning techniques.
Along with the release of more open-source blood cell datasets, automatic cell classification and counting techniques have been proposed, including the traditional image processing and machine learning based methods, as well as the deep learning based frameworks.

\textbf{Traditional methods.} 
% Image processing approaches mainly involve segmentation, feature extraction, classification, and counting steps.
% Alomari et al. \cite{alomari2014automatic} used the Circular Hough Transform (CHT) algorithm with multi-iteration to classify and count RBCs.
% But the above methods based on the Hough Transform have the following disadvantages: (1) These methods have high time and space complexity and low recognition efficiency. (2) These methods can only process simple cell images, and their performance is significantly reduced when processing complex blood cell images.
Generally, cell classification using traditional image processing and machine learning techniques involves image segmentation, feature extraction, classification, and counting steps.
For example, Alomari et al. \cite{alomari2014automatic} employed the Circular Hough Transform (CHT) in an iterative circle detection framework to segment, classify and count WBCs and RBCs.
Such hough transform based shape detection methods are usually time-consuming and their detection and classification accuracy may be significantly reduced when the shape of the blood cells becomes more complex.
% %
% Concurrently, machine learning methods have been applied to blood cell classification and counting.
% Lippeveld et al. \cite{lippeveld2020classification} used the machine learning techniques such as random forest (RF)\cite{breiman2001random} and gradient boosting (GB) classifier \cite{friedman2002stochastic} to classify and count the stain-free WBCs images.
% Tavakoli et al. \cite{tavakoli2021new} proposed a new segmentation and feature extraction algorithm for classifying WBCs images. They presented to construct feature vectors using the cell's shape and color information.
% Sajad et al.\cite{tavakoli2021generalizability} also utilized the shape and color information of WBCs to complete classification and counting. Furthermore, they believed that such information could improve the generalization of the machine learning models to different cell datasets.
% Petrovi et al. \cite{petrovic2020sickle} aimed to address the classification of RBCs in sickle-cell disease. Three features (texture, shape, and color) are manually designed and then the Random Search\cite{bergstra2012random} is exploited to determine the optimal parameters of machine learning models such as SVM\cite{cortes1995support}, KNN\cite{altman1992introduction}, and so on. 
% However, most machine-learning-based algorithms suffer from one problem: heavy pre-processing work. Researchers have to design the feature vectors manually, and the model's performance will depend heavily on the quality of the feature vectors.
Meanwhile, machine learning based methods aim to classify the blood cells based on some features (e.g., shape and color) extracted from the cell images.
Lippeveld et al. \cite{lippeveld2020classification} applied the traditional machine learning techniques such as random forest \cite{breiman2001random} and gradient boosting classifier \cite{friedman2002stochastic} to classify and count the stain-free WBCs images \rui{based on the size, location, texture, and signal strength feature}.
Tavakoli et al. \cite{tavakoli2021new} proposed a new segmentation and feature extraction algorithm which computes three shape features and four novel color features for classifying WBC images.
Although above traditional methods have achieved appealing results for WBC or RBC classification on certain datasets such as Raabin-WBC and LISC, they heavily rely on hand-crafted features which are hardly generalizable to more challenging tasks, e.g., fine-grained classification on our BMEC.   

\textbf{Deep learning based cell classification.}
%Deep learning can automatically extract features to complete classification tasks instead of designing them manually. Such techniques mainly apply the pre-trained CNN models to classify and count the blood cell images.
Deep learning can automatically extract features by learning from a large amount of data to compute tasks such as classification and detection.
To apply deep learning models for the cell classification, one way is to use models pre-trained on general large image datasets for feature extraction and perform particular traditional feature selection and classification methods on the smaller-scale WBC or RBC dataset.
In \cite{tougaccar2020classification}, features extracted from pre-trained AlexNet \cite{krizhevsky2012imagenet}, GoogLeNet \cite{szegedy2015going} and ResNet50 \cite{he2016deep} models are filtered using the Maximal Information Coefficient and Ridge feature selection methods, and quadratic discriminant analysis was used as a classifier on a dataset of WBCs.
Sahlol et al. \cite{sahlol2020efficient} employed a statistically enhanced Salp Swarm Algorithm\cite{mirjalili2017salp} to filter the features extracted from WBC images using the VGG \cite{simonyan2014very} model pre-trained on ImageNet and performed the classification using a traditional decision tree.

\begin{figure*}[!t]
    \centering
    \includegraphics[scale=0.65]{fig/cell_show (1).png}
    \caption{ Full-field erythroid cell image and  four different types of erythroid cells in BMEC cropped by manually annotated ROI: proerythroblast (Pro), basophilic erythroblast (Bas), polychromatophilic erythroblast (Pol), and Orthochromic erythroblast (Ort).
    }
    \label{fig:cell_type}
\end{figure*}


The other way to apply deep learning for cell classification is using the transfer learning technique which starts from a pre-trained CNN model and performs model fine-tuning on a specific WBC or RBC dataset.
For example, Alzubaidi et al. \cite{alzubaidi2020deep} first trained a CNN model on a combination of three WBC datasets and then employed transfer learning to classify RBC images in erythrocytesIDB \cite{gonzalez2014red}.
% Banik et al. \cite{banik2020automatic} presented a new convolutional neural network (CNN) model by fusing the features of the first and last convolutional layers \ruim{[Rui: more details, do they use transfer learning or only use the model for feature extraction and then do traditional feature selection?]}. 
\wy{
Pasupa et al. \cite{pasupa2020convolutional} exploited pre-trained ResNet \cite{he2016deep} and DenseNet \cite{huang2017densely} and performed fine-tuning on their RBC images. In addition, they have handled the class imbalance problem by incorporating the focal loss \cite{lin2017focal}
}.
Comparing to traditional machine learning techniques, deep learning based classification methods can achieve superior performance without manual feature design. 
However, it is difficult to either train a traditional classifier or perform transfer learning for the fine-grained classification task, especially when there is no sufficient finely annotated training data.
We propose a novel shape-aware transfer learning framework that utilizes different types of pre-trained backbone models and fine-tunes the network on our large-scale BMEC for fine-grained erythroid cell classification.


\textbf{Shape-aware cell classification.}
The cell's morphological or shape characteristics such as the circularity, convexity and size have been investigated in traditional methods \cite{alomari2014automatic, lippeveld2020classification, tavakoli2021new} for cell classification.
For deep learning based methods, given only the original cell images, the networks can automatically learn some shape features \cite{zeiler2014visualizing} which are generally more robust than the hand-crafted ones.
However, the implicit learning of deep shape features requires a large amount of training data.
Even when transfer learning is used, it may be still difficult for the network to learn the fine-grained shape variations.
% (cell nucleus and convex hull derived masks) 
To explicitly incorporate the shape information in the network, Tavakoli et al. \cite{tavakoli2021generalizability} passed two binary shape images along with the RGB images of WBCs to a customized CNN with five channels (three for RGB and two for shape masks) and showed the generalizability of the model can be improved when the shape masks are used.
Similarly, we also explicitly integrate the shape information into the network.
Instead of using the nucleus and ROC (Representative Of
the Convex hull = convex hull - nucleus) images as in \cite{tavakoli2021generalizability}, we choose convex hull as our shape mask image since we find the contour is more suitable to represent the shape of erythroid cells.
Moreover, we design a novel shape attention module which computes a shape-attended image feature, to improve the learning of fine-grained shape-aware image features.



==> 03BMEC.tex <==


\section{BMEC Dataset}

% This section will discuss the BMEC dataset collected by us and the approach used in this paper.
% The BMEC dataset includes four types of erythroid cells: proerythroblast(Pro), basophilic erythroblast(Bas), polychromatophilic erythroblast(Pol), and orthochromic erythrobla(Ort).
% Our method mainly consists of four modules which are cell shape extraction, dual branch network, shape attention module and feature fusion module. 
% The workflow of our approach is shown in Figure 1.

% \subsection{BMEC Dataset}
Our BMEC dataset was built based on the data acquired at the Second Hospital of Jilin University, Changchun, China. 
It contains 5,666 erythroid cell images which are annotated into four fine-grained types by three hematologists.
The shape differences between the types are subtle, which makes the classification on BMEC more challenging than existing WBC datasets or RBC datasets with abnormal erythroid cells.
% This dataset contains  four  types  of  erythroid cells: proerythroblast (Pro),  basophilic erythroblast (Bas),  polychromatophilic erythroblast (Pol), and orthochromic erythrobla (Ort). 
% We collected 239 sets of bone marrow erythroid cell smears from 128 patients. 


\begin{table}[h]
\begin{center}
\begin{minipage}{210pt}
\caption{The characteristics of different erythroid cells summarized in \cite{gregory2001bigger}. }\label{tab:chara}%

\begin{tabular}{@{}llll@{}}
\toprule
Cells  & Percent\footnotemark[1]  & Diameter & Shape\\
\midrule
Pro   & 0.5\%-4\% & 15um-20um & elliptical, protrusions \\
Bas   & 1\%-5\%   & 10um-18um & round, protrusions      \\
Pol   & 12\%-20\% & 8um-15um  & round, rough edges      \\
Ort   & 6\%-12\%  & 7um-10um  & round, smooth edges     \\
\botrule
\end{tabular}
\footnotetext[1]{The Percent column indicates the percentage of the corresponding cell type in all types of bone marrow cells, including both WBC and erythroid.}
% \footnotetext[1]{Example for a first table footnote. This is an example of table footnote.}
% \footnotetext[2]{Example for a second table footnote. This is an example of table footnote.}
\end{minipage}
\end{center}
\end{table}



\begin{table}[h]
\begin{center}
\begin{minipage}{\textwidth}
\caption{The statistics of the BMEC dataset in terms of distributions of different cells.}\label{tab:bmec}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccc@{\extracolsep{\fill}}}
\toprule%
% & \multicolumn{6}{@{}c@{}}{BMEC Dataset Statistic} 
% \\\cmidrule{2-7}
Dataset & Quantity & Percent & Pro\footnotemark[1]  & Bas\footnotemark[1] & Pol\footnotemark[1] & Ort\footnotemark[1] \\
\midrule
Training Set.   & 3,865& 68.2\%  & 146(2.6\%) & 428(7.6\%) & 1,702(30.0\%) & 1,589(28.0\%)\\
Validation Set  & 655  & 11.6\%  & 28(0.5\%)  & 69(1.2\%)  & 312(5.5\%)    & 246(4.4\%)\\
Test Set        & 1,146& 20.2\%  & 48(0.8\%)  & 115(2.0\%) & 526(9.3\%)    & 457(8.1\%)\\
Total           & 5,666& 100\%   & 222(3.9\%) & 612(10.8\%)& 2,540(44.8\%) & 2,292(40.5\%)\\
\botrule
\end{tabular*}
\footnotetext[1]{proerythroblast cells (Pro), basophilic erythroblast cells (Bas), polychromatophilic erythroblast cells (Pol), orthochromic erythrobla cells (Ort).}

\end{minipage}
\end{center}
\end{table}


% \begin{table*}[]
% \centering
% \begin{tabular}{|c|c|c|cccc|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}BMEC\\ Dataset\end{tabular}} & \multirow{2}{*}{Quantity} & \multirow{2}{*}{Percent} & \multicolumn{4}{c|}{No. and Percent of Cells}                                                   \\ \cline{4-7} 
%                                                                         &                       &                          & \multicolumn{1}{c|}{Pro} & \multicolumn{1}{c|}{Bas} & \multicolumn{1}{c|}{Pol}  & Ort  \\ \hline
% Training Set                                                            & 3,865                  & 68.2\%                     & \multicolumn{1}{c|}{146 (2.6\%)} & \multicolumn{1}{c|}{428 (7.6\%)} & \multicolumn{1}{c|}{1,702 (30.0\%)} & 1,589 (28.0\%) \\ \hline
% Validation set                                                          & 655                   & 11.6\%                     & \multicolumn{1}{c|}{28 (0.5\%)}  & \multicolumn{1}{c|}{69 (1.2\%)}  & \multicolumn{1}{c|}{312 (5.5\%)}  & 246 (4.4\%)  \\ \hline
% Test Set                                                                & 1,146                  & 20.2\%                     & \multicolumn{1}{c|}{48 (0.8\%)}  & \multicolumn{1}{c|}{115 (2.0\%)} & \multicolumn{1}{c|}{526 (9.3\%)}  & 457 (8.1\%) \\ \hline
% Total                                                                & 5,666                  & 100\%                     & \multicolumn{1}{c|}{222 (3.9\%)}  & \multicolumn{1}{c|}{612 (10.8\%)} & \multicolumn{1}{c|}{2,540 (44.8\%)}  & 2,292 (40.5\%)  \\ \hline

% \end{tabular}
% \caption{The statistics of the BMEC dataset in terms of distributions of different cells.}
% \label{tab:bmec}
% \end{table*}

\textbf{Smears Imaging and Cell Extraction.}
The original data contains 239 sets of bone marrow erythroid cell smears collected from 128 patients using the BEION V4.90 system between 2019 and 2021.
To meet the requirements of clinical evaluation and diagnosis, each smear contains more than 200 blood cells.
In the collection process, the hematologist first stained all smears using the Richter stain method.
Then, the observation of an Olympus BX43 microscope at 100X magnification was captured into images of 2592 $\times$ 1944 resolution.

To extract individual erythroid cells from the smear images, two experienced hematologists worked together to select a  ROI (region of interest) for each cell and crop the selections into cell images (Figure \ref{fig:cell_type}).
When extracting the cells, the hematologists mainly follow two principles: 1) not introduce too much background and noise; 2) preserve the whole cell shape to the maximum extent.
%When one hematologist has completed the cropping, another hematologist will examine the cropping results, which can filter out other cells that do not belong to the erythroid cells.
When one hematologist completed the cropping, the other hematologist examined the results to ensure the quality of the extracted images, e.g., no other cells rather except the central erythroid cell appear in the image.
In the end, 5,666 erythroid cell images are extracted from the blood smears.
Each cell image is resized to 224$\times$224 resolution.
%These cells mainly consist of four types of erythroid cells: Pro, Bas, Pol, and Ort.


\textbf{Data Annotation.}
Based on the growth and maturation, the erythroid cells are annotated into four types (Figure \ref{fig:cell_type} right):
proerythroblast (Pro), basophilic erythroblast (Bas), polychromatophilic erythroblast (Pol), and orthochromic erythrobla (Ort).
Note that we only focus on the erythroid cells which have normal shapes and do not consider the abnormal erythroid cells with elongated shapes such as in erythrocytesIDB \cite{gonzalez2014red}.
\rui{For reference, in Table \ref{tab:chara}, we show the characteristics (e.g., percentage, size and shape) summarized in \cite{gregory2001bigger}, for the four types of erythroid cells.}

As the shape differences of the collected erythroid cells are indeed very subtle, to reduce the subjectiveness in annotation, we invited three hematologists and designed a rigorous annotation process to obtain more consistent labels.
% Firstly, the first hematologists annotates all cell images. At the same time, the second hematologist also annotates all cell images, the two annotation processes being independent and unknown to each other.
First, two hematologists independently annotated all the cell images without any interference.
The annotation results of the two hematologists were compared and the cell images with different assigned labels were re-annotated by the two hematologists for the second pass.  
If the re-annotation results were still different, the third hematologist would provide another annotation on these images, and the final cell category would be determined by voting the annotations from the three hematologists.
%Such a labeling process is very rigorous, and it eliminates the errors caused by subjective differences.

\textbf{Statistics.}
As shown in Table \ref{tab:bmec}, we divide the BMEC dataset into a training set, a validation set and a test set with an approximate ratio of 7:1:2.
It can be observed that for each set, the percentage of the four cell types follows the relative cell distribution mentioned in Table \ref{tab:chara}, e.g., the number of Pol is about four times of Bas.

% \begin{table}[h!t]
% % \setlength{\tabcolsep}{1mm}{
% \begin{tabular}{|c|c|c|cccc|}
% \hline
% \multirow{}{}{BMEC Dataset} & \multirow{}{}{Size} & \multirow{}{}{Percent} & \multicolumn{4}{c|}{Numbers of cells}                                                  \\ \cline{4-7} 
%          &      &      & \multicolumn{1}{c|}{Pro} & \multicolumn{1}{c|}{Bas} & \multicolumn{1}{c|}{Pol}  & Ort  \\ \hline
% Training Set                  & 4520                  & 80\%                     & \multicolumn{1}{c|}{174} & \multicolumn{1}{c|}{497} & \multicolumn{1}{c|}{2014} & 1835 \\ \hline
% Test Set & 1146 & 10\% & \multicolumn{1}{c|}{48}  & \multicolumn{1}{c|}{115} & \multicolumn{1}{c|}{526}  & 457  \\ \hline
% Total    & 5,666 & -    & \multicolumn{1}{c|}{222} & \multicolumn{1}{c|}{612} & \multicolumn{1}{c|}{2540} & 2292 \\ \hline
% \end{tabular}
% % }
% \caption{The details of the BMEC dataset in terms of percentages and distributions of different cells.}
% \label{tab:my-table_cells}
% \end{table}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}



% if the results of the two experts are different, the image will be renegotiated by them to give a consistent labeling result.
% Figure 2 shows the sample images and Table 2 presents the details of the datasets in terms of percentages and distributions of different classes.


% As shown in Table \ref{tab:chara} and Figure \ref{fig:cell_type}, we compare the characters of four types of erythroid cells in detail.
% The Percent column indicates the percentage of this cell in the total number of bone marrow cells.
% The Diameter column represents the diameter of this cell.
% The Shape column describes the shape and contour characteristics of this cell. We can find that there are some differences in terms of shape and diameter between erythroid cells.



% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% \begin{table}[hit]\normalsize
% \setlength{\tabcolsep}{}{
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% Cell & Percent(\%)   & Diameter(um)  & Shape                            & Nucleus Size   \\ \hline
% Pro   & 0.5-4 & 15-20 & elliptical, protrusions & 0.8            \\ \hline
% Bas   & 1-5   & 10-18 & round, protrusions      & 0.6            \\ \hline
% Pol   & 12-20 & 8-15  & round, rough edges      & 0.5            \\ \hline
% Ort   & 6-12  & 7-10  & round, smooth edges     & \textless{}0.5 \\ \hline
% \end{tabular}
% }

% \caption{we compare the characters of four types of erythroid cells in detail.
% The Percent col indicates the percentage of this cell in the total number of bone marrow cells.
% The Diameter col represents the diameter of this cell.
% The Shape col describes the shape and contour information of this cell.
% The Nucleus Size col means the cell's nucleus size.
% }
% \label{tab:my-table_cell_characters}
% \end{table}






% The most important characteristics of the BMEC dataset that discriminates it from other blood cell datasets are as follows:

% \begin{itemize}
% \item \textbf{The first erythroid cell dataset}:
% BMEC dataset is the first dataset on erythroid cells and it contains four types of erythroid cells, including Pro,  Bas, Pol, and Ort.  
% \item  \textbf{large number of cells}: As shown in Table \ref{tab:bmec}, we collected a total of 5,666 cell images. 
% BMEC is a relatively large dataset compared to other cell datasets, as shown in Table \ref{tab:datasets}.
% \item \textbf{Triple Check}: All images in the BMEC dataset were checked three times, which eliminates subjective differences and provides more accurate labels.


% \item \textbf{Free public access}: Since we aim at supporting the research on erythroid cells classification, the BMEC dataset is freely available for all.
% \end{itemize}

In the following, we summarize the key characteristics that discriminate our BMEC dataset from other blood cell datasets:

\begin{itemize}
\item \textbf{The first fine-grained erythroid cell dataset.}
BMEC dataset is the first dataset that contains four fine-grained types of normal erythroid cells: Pro,  Bas, Pol, and Ort. It is more challenging than existing WBC or erythroid cell datasets since the shape differences between the types are subtle.
\item  \textbf{Largest number of erythroid cells}. As shown in Table \ref{tab:datasets},
BMEC is currently the largest dataset for erythroid cells, which is expected to enable more deep learning research on erythroid cells.
\item \textbf{Professional and rigorous annotation}. The images in the BMEC dataset were professionally annotated by three hematologists following a rigorous labeling process, which reduces the subjectiveness and ensures the quality of the annotation.
\item \textbf{Free public access}. We make the BMEC dataset freely available for all communities, with the hope that it can inspire more follow-ups research on erythroid cells.
\end{itemize}



==> 04methods.tex <==

\begin{figure*}[h!t]
    % \centering
    \includegraphics[scale=0.55]{fig/dual_branch_network (6).png}
    \caption{The overview of our approach. The novel shape attention module calculates a shape-attended image feature using the raw and shape features ($\otimes$ represents the broadcasted element-wise matrix multiplication operation). The fused shape-aware feature is used for the final fine-grained classification.  
    }
    \label{fig:overview}
\end{figure*}


\section{Method}
% The objective of our work is to improve erythroid cells classification by harnessing the shape information of erythroid cells.

% To accomplish this task, we consider RGB cell images and binary cell images data as $X = \{x_R^i,X_S^i\}_{i=1}^n $ and labels as $Y=\{ y^i\}_{i=1}^n$.
% Here, $x_R^i \in R^{M\times N \times C_1}$ and $X_S^i \in R^{M\times N \times C_2}$, $C_1$ and $C_2$ denote the number of channels in RGB cell images and binary cell images respectively, while $n$ denote the number of samples.


\subsection{Overview}
% This research work aims to utilize the shape and size properties of erythroid cells to improve classification accuracy. 

% As shown in Figure \ref{fig:overview}, this is achieved in three steps: firstly, the shape information of cells is extracted and saved as binary images from RGB cell images. Secondly, the binary images and RGB images are sent to feature extraction networks to obtain raw feature and shape feature, and then the shape feature is passed through the shape attention module to calculate shape attention weights, which are harnessed to enhance the latent shape feature from RGB images. Finally, we fuse these features to obtain hybrid features and complete the classification.

Our pipeline consists of four modules as shown in Figure \ref{fig:overview}: a cell shape extraction module, a dual-branch network, a shape attention module and a cell classification network.
The shape extraction module transforms the RGB erythroid cell image into the binary shape mask. The RGB image and shape mask are separately passed to the dual-branch network to generate the raw and shape features. The shape attention module calculates the shape attention weights and generates a shape-attended image feature from the raw image feature.
Then, the raw image feature, shape-attended image feature and the shape feature are aggregated to a fused shape-aware feature, which is passed to the lightweight classification network for prediction.

\begin{algorithm}
\caption{The cell segmentation pipeline following \cite{tavakoli2021new}}\label{algo1}
\begin{algorithmic}[1]
\State Input RGB erythroid cell image 

\State Convert the input RGB image to CMYK color space 
\label{ code:fram:extract }
\State Calculate $KM = (K\_component) - (M\_component)$
\label{code:fram:trainbase}
% \STATE Convert  the RGB input image to HLS color space
% \label{code:fram:add}
\State Convert  the RGB input image to HLS color space and calculate $MS = Min(M\_component, S\_component)$
\label{code:fram:classify}
\State Calculate $V  = MS - KM$
\label{code:fram:select}
\State Exploit Otsu's thresholding algorithm \cite{NobuyukiOtsu1979ATS} to segment the cell and obtain the cell nucleus $N$
\State Calculate the convex hull of the cell to acquire the shape mask $S$ based on $N$
\State Calculate the cell cytoplasm $C = S - N$ 
% \ruim{[Rui: for 7,8,9, all three steps use Otsu's thresholding?? What is the targe image in 7,8,9? Add reference for Otsu's thresholding.]}
\State Output the convex hull $S$, nucleus $N$, cytoplasm $C$ as the binary segmentation masks
\end{algorithmic}
\end{algorithm}

% \begin{algorithm*}[htb]
% \centering
% \caption{ The cell segmentation pipeline following \cite{tavakoli2021new}} 
% \label{alg:Framwork} 
% \begin{algorithmic}[1] %这个1 表示每一行都显示数字
% % \REQUIRE ~~\\ %算法的输入参数：Input
% % The set of positive samples for current batch, $P_n$;\\
% % The set of unlabelled samples for current batch, $U_n$;\\
% % Ensemble of classifiers on former batches, $E_{n-1}$;
% % \ENSURE ~~\\ %算法的输出：Output
% % Ensemble of classifiers on the current batch, $E_n$;
% \STATE Input RGB erythroid cell image
% \STATE Convert the input RGB image to CMYK color space 
% \label{ code:fram:extract }
% \STATE Calculate $KM = (K\_component) - (M\_component)$
% \label{code:fram:trainbase}
% % \STATE Convert  the RGB input image to HLS color space
% % \label{code:fram:add}
% \STATE Convert  the RGB input image to HLS color space and calculate $MS = Min(M\_component, S\_component)$
% \label{code:fram:classify}
% \STATE Calculate $V  = MS - KM$
% \label{code:fram:select}
% \STATE Exploit Otsu's thresholding algorithm \cite{NobuyukiOtsu1979ATS} to segment the cell and obtain the cell nucleus $N$
% \STATE Calculate the convex hull of the cell to acquire the shape mask $S$ based on $N$
% \STATE Calculate the cell cytoplasm $C = S - N$ 
% % \ruim{[Rui: for 7,8,9, all three steps use Otsu's thresholding?? What is the targe image in 7,8,9? Add reference for Otsu's thresholding.]}
% \STATE Output the convex hull $S$, nucleus $N$, cytoplasm $C$ as the binary segmentation masks
% \label{code:ostu}
% \end{algorithmic}
% \end{algorithm*}

\subsection{Cell Shape Extraction}
% During the growth and development of erythroid cells, the cell diameter gradually decreases. 
%As shown in Table \ref{tab:chara} and Figure \ref{fig:cell_type}, erythroid cells at different maturity stages are different in cell shape. And more importantly, the shape information can increase the interclass distance and thus improve the classification accuracy. \textcolor{wy}{Therefore, we want to explicitly extract information about erythroid cell shape and treat it as a priori knowledge for the model. This is our idea and initial intention to design the module. }
%We refer to and use the cell segmentation method in this work\cite{tavakoli2021new} to extract the cell shape of our dataset.

From Figure \ref{fig:cell_type} and Table \ref{tab:chara}, it can be observed the shape information is crucial to distinguish different fine-grained types of erythroid cells, especially when the appearances of the cells are similar.
Therefore, we explicitly extract the cell shape information as a binary shape mask and treat it as a prior knowledge (or inductive bias) for the classification model. 
We employ the cell image segmentation method proposed in \cite{tavakoli2021new} to extract the shape mask for each BMEC cell image.
The main steps of cell shape extraction are shown in Algorithm \ref{alg:Framwork}, while Figure \ref{fig:interm} shows the corresponding intermediate and segmentation results.
Three types of binary mask images are obtained: the convex hull, nucleus and cytoplasm.
Figure \ref{fig:seg_results} shows the image segmentation results of different types of erythroid cells.

Unlike \cite{tavakoli2021generalizability} which utilized the nucleus and ROC (convex hull - nucleus) images as the shape images, we choose the convex hull image as our shape image.
The main reason is \cite{tavakoli2021generalizability} mainly focuses on the WBCs whose nucleuses are in apparently different shapes.
However, for erythroid cells, their nucleuses are more intact and look quite similar comparing to WBCs (see Figure \ref{fig:seg_results}).
Also, the cytoplasm (i.e., the ROC in \cite{tavakoli2021generalizability}) images of the erythroid cells are noisy and not suitable to represent the cell shapes.
In contrast, convex hull contains the key shape characteristics and it is more robust to noise comparing to the nucleus.
We pass the binary image of convex hull to our network and also compute the shape attention to enhance the original image feature.


\begin{figure*}[h!t]
    \centering
    \includegraphics[scale=0.5]{fig/分割效果流程图 (6).png}
    \caption{ The results obtained by applying different steps of Algorithm 1. 
    }
    \label{fig:interm}
\end{figure*}

% \begin{enumerate}
%     \item Converting erythroid cell images to CMYK color space
%     \item Calculating  KM = (K component) - (M component)
%     \item Converting erythroid cell images to HLS color space
%     \item Calculating  MS = Min(M component, S component)
%     \item Calculating  V = MS - KM
%     \item Exploiting Otsu’s thresholding algorithm to segment the cell
% \end{enumerate}



% The results of erythroid cell images segmentation using this method are shown in Figure \ref{fig:seg_results}.
% We can get three types of binary images: shape and contour image, nucleus image, and cytoplasm image. 
% We suppose that the shape and contour image is more important than the other two images.
% The reasons are as follows:

% \begin{itemize}
% \item Different stages of erythroid cells differ in shape, and these differences are significant for cell classification. The shape and contour image is a good representation of the shape of cells, and it can reflect the differences between different erythroid cells.
% \item The information provided by the cytoplasm image is not enough to improve cell classification.
% \item The nucleus image contains too many unrelated details, which cannot benefit erythroid cell classification.
% \end{itemize} 

\begin{figure*}[h!t]
    \centering
    \includegraphics[scale=0.5]{fig/cell_show_2_rows (3).png}
    \caption{ This figure shows the RGB images and other segmentation results (Nucleus mask, Shape mask, and Cytoplasm mask) of four types of erythroid cells.
    } 
    \label{fig:seg_results}
\end{figure*}

% As shown in Figure \ref{fig:seg_results}, these four types of cells are very similar in raw RGB images (especially between Pro, Bas, and Pol).
% However, in the second row images, we observe distinct differences in terms of shape and size. 
% We consider that such differences are essential for erythroid cells classification.
% Therefore, we extract the shape information as a binary image from the RGB erythroid cell image and use it as input to the DBN module.



\subsection{Dual-Branch Network}
To explicitly integrate the shape information into the deep learning framework, we design a dual-branch network which encodes the RGB image and the binary shape mask (convex hull image) in two separate branches.

As shown in Figure \ref{fig:overview}, the top branch network takes the RGB image as input and extracts the raw feature using Swin-Transformer \cite{liu2021swin}, the state-of-the-art backbone model for image feature extraction.
Although the RGB image branch can learn the pixel intensity variations between different cells, it does not focus on the cell's shape or structure characteristics.
Therefore, we introduce a separate bottom branch network which employs a VGG19 \cite{he2016deep} model to explicitly compute the shape feature from the binary shape mask image obtained from the cell shape extraction module.
The raw image feature and the shape feature from two branches are integrated in the shape attention module (Section \ref{sec:shape_att}) and fused in the later stage.
In Section \ref{sec:ablation}, we show the shape branch is an effective complement to the RGB branch for fine-grained cell classification.
In addition, our dual-branch network is a general design such that the backbone models in each branch can be replaced by other deep image feature extraction models.
In current our experiments, we find using the combination of Swin-Transformer and VGG19 for the two branches can achieve the best performance (Table \ref{tab:backbone_top} and \ref{tab:backbone_bottom}).


% \begin{table*}[h!t]
% % \centering

% \begin{tabular}{|c|c|c|c|c|}
% \hline
%  Top branch network                             & Down branch network & Inputs    & Mean Acc & Acc Range \\ \hline
% \multirow{}{}{ResNet18\cite{he2016deep}}        & ---  & RGB        &  79.18\% & 78.53\%-79.67\%  \\ \cline{2-5} 
%                                 & VGG19\cite{simonyan2014very}  & RGB+Shape         & 79.95\% & 79.79\%-80.14\% \\ \hline
% \multirow{}{}{ResNet50\cite{he2016deep}}         & ---  & RGB       &      79.31\%  & 78.92\%-79.79\%  \\\cline{2-5} 
%                                 & VGG19\cite{simonyan2014very}  & RGB+Shape &    79.91\% & 79.44\%-80.40\%  \\ \hline
% \multirow{}{}{DenseNet121\cite{huang2017densely}}    & ---  & RGB       &       79.25\%  & 78.71\%-79.76\% \\ \cline{2-5} 
%                                 & VGG19\cite{simonyan2014very}  & RGB+Shape &    80.65\%  & 80.05\%-81.02\% \\ \hline
% \multirow{}{}{ResNest\cite{HangZhang2020ResNeStSN}}  & --- & RGB       &      80.88\%  & 80.36\%-81.15\% \\ \cline{2-5} 
%                                 & VGG19\cite{simonyan2014very}  & RGB+Shape &   81.15\% & 80.66\%-81.62\% \\ \hline
% \multirow{}{}{Swin-Transformer\cite{liu2021swin}} & --- & RGB       &      80.68\% & 80.19\%-81.15\% \\ \cline{2-5} 
%                             & VGG19\cite{simonyan2014very}      & RGB+Shape &    \textbf{82.03\%} & \textbf{81.89\%-82.15\%} \\ \hline
                                  
% % \row{Swin-Transformer+Attention}                   & Raw+Shape & \checkmark & 82.03\% &81.89\%-82.15\% \\ \hline
% \end{tabular}
% \caption{Compare the effect of using the shape attention module on different models. 
% For each model and each set of inputs, we take the average result of 5 experiments as the final accuracy to eliminate the experimental fluctuations.
% \textcolor{wy}{When the input is RGB image , we just employ the top branch network to complete the classification directly.
% When the input is RGB image and Shape image, we utilize the two-branch network and combine it with the shape attention module to complete the classification.}
% }
% \label{tab:my-table}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}





\subsection{Shape Attention}
\label{sec:shape_att}
% As shown in Figure \ref{fig:overview}, the Feature Extraction Networks extracted feature maps from two types of images. The feature map from the shape mask is sent to Shape Attention module to learn shape attention weights, which are harnessed to enhance the latent shape features from the RGB images.
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[scale=0.5]{cross_attention (3).png}
%     \caption{ (a): The attention mechanism in SENet\cite{JieHu2018SqueezeandExcitationN}.
%     (b): The workflow of Shape Attention module proposed by this work. 
%     (c): The network architecture of Shape Attention module . 
%     }
%     \label{fig_5}
% \end{figure}


% The Shape Attention module proposed by this work is different from the attention mechanism in SENet\cite{JieHu2018SqueezeandExcitationN}. SENet works only on single input where both the hidden representations as well as the attention weights are derived from the same input. However, our Shape Attention module calculates attention weights from the shape mask and obtains a shape-attended image feature. Therefore, our Shape Attention module can extract multi-view features by crossing different inputs.
% As shown in Figure \ref{fig:overview}, this module contains just two fully connected layers and two activation functions. Therefore, it is a very lightweight network.

To further integrate the shape information to the extracted image feature, we propose a novel shape attention module which takes the raw image feature and shape feature as input and outputs a shape-attended image feature (see Figure \ref{fig:overview} middle).
First, the shape attention weights are computed from the binary shape mask image following the similar attention mechanism used in SENet \cite{JieHu2018SqueezeandExcitationN}.
Then, the raw image feature is multiplied by the shape attention weights to get the shape-attended feature.
The mathematical formulation is as follows:

% SatyamMohla2020FusAtNetDA
\begin{equation}
\label{eq:fr}
    F_R = Swin-Transformer(X_R),
\end{equation}
\begin{equation}
\label{eq:fs}
    F_S = VGG19(X_S),
\end{equation}
\begin{equation}
\label{eq:wa}
    W_{SA} = Sigmoid(W_2(ReLU(W_1(F_S)))),
\end{equation}
\begin{equation}
\label{eq:fa}
    F_{SA} = W_{SA}\otimes F_R.
\end{equation}
\\


% We consider RGB cell images and binary shape images data as $X = \{x_R^i,X_S^i\}_{i=1}^n $ and labels as $Y=\{ y^i\}_{i=1}^n$.
% Here, $x_R^i \in R^{M\times N \times C_1}$ and $X_S^i \in R^{M\times N \times C_2}$, $C_1$ and $C_2$ denote the number of channels in RGB cell images and shape mask respectively, while $n$ denote the number of samples.

% As shown in Equation \ref{eq:fr} and \ref{eq:fs}, we define the outputs of Swin-Transformer \cite{liu2021swin} and VGG19\cite{simonyan2014very} as $F_R$, $F_S$, respectively.
% $F_S$, the shape feature of cells, is sent to the SA module.
% As shown in Equations 3, 4 and Figure \ref{fig:seg_results} (b), (c), it is first sent to the first fully connected layer ($FC_1$), and then the output of $FC_1$ is activated by the Relu layer ($ReLU$).
% The output of $ReLU$ is transmitted to the second fully connected layer ($FC_2$), and finally, the shape attention weights ($W_{SA}$) are obtained by activating the sigmoid layer. 
% The latent shape feature in $F_R$ can be enhanced by multiplying shape attention weights ($W_{SA}$) as shown in Equation 4.

\noindent Here, $X_R \in R^{224\times 224 \times 3}$ and $X_S \in R^{224\times 224 \times 1}$ are the input RGB image and binary shape mask, respectively;
$F_R$ and $F_S$ are the corresponding features extracted using Swin-Transformer \cite{liu2021swin} and VGG19 \cite{simonyan2014very}.
As shown in Equation \ref{eq:wa} and Figure \ref{fig:overview}, the shape attention weights $W_{SA}$ are calculated by passing $F_S$ through two fully connected layers ($W_1$ and $W_2$) which are followed by a ReLU and a Sigmoid layer, respectively.
Finally, the shape-attended feature $F_{SA}$ is obtained by performing element-wise multiplication of the shape attention weights $W_{SA}$ and the raw image feature $F_R$.
In summary, the shape attention module is a lightweight network that can efficiently computes the correlation among the shape feature and enhances the raw image feature with self-learned cell shape information.
Moreover, the shape attention module can be combined with any backbone models to integrate the shape information to the image feature.

% Here, three features are obtained, which are $F_R$, $F_S$, and $F_{SA}$.
% $F_R$, the output of Swin-Transformer\cite{liu2021swin}, contains plenty of raw features such as color and texture features. 
% However, the shape features are not apparent in $F_R$.
% In $F_S$, no color or texture information is included. But it contains information about the shape of erythroid cells.
% The shape attention weights ($W_{SA}$) indicate the correlation of the shape information at different locations in the form of probabilities.
% Therefore, the latent shape in $F_R$ can be enhanced by multiplying $W_{SA}$.
% At last, these three feature maps are joined to form information-rich hybrid features, as shown in Equation 5.


\subsection{Cell Classification Network}
The last module of our pipeline is a conventional classification network which consists of two sets of fully connected, ReLu and Dropout layers (Figure \ref{fig:overview} right).
The raw image feature $F_R$, shape feature $F_S$ and shape-attended image feature $F_{SA}$ are concatenated to form an fused cell feature $F_C = \{F_R, F_{SA}, F_S\}$ for final classification. 
% The hybrid features contain three features, which are $F_R$, $F_S$, and $F_{SA}$, respectively. We design a relatively simple network for learning the hybrid features and accomplishing to classify. \textcolor{raw}{As shown in Figure \ref{fig:overview}, this model consists of three fully connected layers, two Relu layers, and two Dropout layers.}
With the shape feature and shape attention explicitly considered, the shape-aware network can achieve superior performance comparing to only using the RGB feature for the fine-grained erythroid cell classification (see Table \ref{tab:ablation}).





% \begin{table*}[htbp]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% Top branch  network                      & bottom branch  network    & Inputs    & Accuracy & Precision & Recall  & F1      \\ \hline
% \multirow{4}{*}{Swin-Transformer \cite{liu2021swin}} 
%                                   & ResNet18 \cite{he2016deep}         & RGB+Shape & 80.62\%  & 78.68\%   & 74.93\% & 73.23\% \\ \cline{2-7} 
%                                   & ResNet50 \cite{he2016deep}         & RGB+Shape & 80.45\%  & 75.44\%   & \textbf{76.21\%} & 72.68\% \\ \cline{2-7} 
%                                   & Swin-Transformer \cite{liu2021swin} & RGB+Shape & 80.36\%         & \textbf{77.45\%}          & 75.81\%        & 73.33\%        \\ \cline{2-7} 
%                                   & VGG19 \cite{simonyan2014very}            & RGB+Shape & \textbf{81.12\%}  & 76.28\%   & 75.73\% & \textbf{74.00\%} \\ \hline
% \end{tabular}      
% \caption{Comparison of different bottom branch backbone networks for classification on BMEC. The top branch network is fixed as Swin-Transformer.}
% \label{tab:backbone_bottom}
% \end{table*}


% \begin{table*}[h!t]
% \centering
% \begin{tabular}{|c|c|c|c|}
% \hline
% Study                          & Method                             & Category Number & Accuracy \\ \hline
% Rezatofighi et al. (2011) \cite{rezatofighi2011automatic} & SVM                               & 5               & 96.00\%  \\ \hline
% Jung et al. (2019) \cite{jung2019w}                      & W-Net based CNN                   & 5               & 97.00\%  \\ \hline

% Baydilli et al. (2020) \cite{baydilli2020classification}              & Capsule Networks        & 5               & 96.86\%  \\ \hline
% Harshanand et al. (2020)  \cite{harshanand2020comprehensive}              & CNN with Swish Activation        & 5               & 97.64\%  \\ \hline
% Tavakoli et al. (2021) \cite{tavakoli2021new}                        & Segmentation                      & 5               & 92.21\%  \\ \hline
% Muhammad et al. (2021) \cite{khan2021automated}            & Feature Selection and ELM        & 4              & 96.60\%  \\ \hline

% Ours                      & Dual-Branch and Shape Attention & 6              & \textbf{98.51\%}    \\ \hline
% \end{tabular}
% \caption{Comparison of different methods for classification on LISC dataset \cite{rezatofighi2011automatic}.
% Due to the data imbalance problem in LISC, other methods directly discarded the cell categories with a low number of images. In contrast, we trained and tested using all categories and still obtained the best accuracy.
% }
% \label{tab:lisc}
% \end{table*}

% \begin{table*}[h!t]
% \centering
% \begin{tabular}{|c|c|c|c|}
% \hline
% Study                          & Method                             & Category Number & Accuracy \\ \hline

% Kumar et al. (2017) \cite{kumar2017automated}            & Color Space Conversion        & 4              & 75.88\%  \\ \hline
% Liang et al. (2018) \cite{GaoboLiang2018CombiningCN}            & Xception-LSTM        & 4              & 90.79\%  \\ \hline
% Pang et al. (2019) \cite{ShuchaoPang2019ANF}            & CNN        & 4              & 90.39\%  \\ \hline

% Partha et al. (2020) \cite{ParthaPratimBanik2020AnAN}            & CNN        & 4              & \textbf{96.00\%}  \\ \hline
% Tavakoli et al. (2021) \cite{tavakoli2021new}            & Segmentation        & 4              & 94.20\%  \\ \hline
% % Muhammad Attique Khan al et. (2021) \cite{khan2021automated}            & Feature selection and ELM        & 4              & 96.60\%  \\ \hline

% Our method                     & Swin-Transformer+Shape Attention & 4           & 95.71\%    \\ \hline
% \end{tabular}
% \caption{Comparison of different methods for classification on BCCD dataset \cite{mohamed2012efficient}.}
% \label{tab:bccd}
% \end{table*}





==> 05experiments.tex <==




\section{Experiments}

\begin{table}[h]
\begin{center}
\begin{minipage}{\textwidth}
\caption{Comparison of different top branch backbone networks for classification on BMEC. The bottom branch network is fixed as VGG19.}\label{tab:backbone_top}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccc@{\extracolsep{\fill}}}
\toprule%
% & \multicolumn{6}{@{}c@{}}{BMEC Dataset Statistic} 
% \\\cmidrule{2-7}
Top & Bottom & Inputs& Acc & Pre& Rec& F1  \\
\midrule
ResNet18 \cite{he2016deep}         & \multirow{5}{*}{VGG19 \cite{simonyan2014very}} & RGB+Shape & 79.51\%  & 74.27\%   & 73.53\% & 72.42\%\\
ResNet50 \cite{he2016deep}         &                        & RGB+Shape & 79.58\%  & 74.33\%   & 73.67\% & 72.51\% \\
DenseNet121 \cite{huang2017densely}      &                        & RGB+Shape & 79.65\%  & 73.42\%   & 73.15\% & 72.20\% \\
ResNest \cite{HangZhang2020ResNeStSN}          &                        & RGB+Shape & 80.12\%  & \textbf{76.47\%}   & 74.64\% & 73.04\% \\
Swin-T \cite{liu2021swin}\footnotemark[1] &                        & RGB+Shape & \textbf{81.12\%}  & 76.28\%   & \textbf{75.73\%} & \textbf{74.00\%} \\


% Validation Set  & 655  & 11.6\%  & 28(0.5\%)  & 69(1.2\%)  & 312(5.5\%)    & 246(4.4\%)\\
% Test Set        & 1,146& 20.2\%  & 48(0.8\%)  & 115(2.0\%) & 526(9.3\%)    & 457(8.1\%)\\
% Total           & 5,666& 100\%   & 222(3.9\%) & 612(10.8\%)& 2,540(44.8\%) & 2,292(40.5\%)\\
\botrule
\end{tabular*}
% \footnotetext[1]{RGB image+Shape Mask image (RGB+S)}
\footnotetext[1]{Swin-Transformer (Swin-T)}

\end{minipage}
\end{center}
\end{table}


\begin{table}[h]
\begin{center}
\begin{minipage}{\textwidth}
\caption{Comparison of different bottom branch backbone networks for classification on BMEC. The top branch network is fixed as Swin-Transformer.}\label{tab:backbone_bottom}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccc@{\extracolsep{\fill}}}
\toprule%
% & \multicolumn{6}{@{}c@{}}{BMEC Dataset Statistic} 
% \\\cmidrule{2-7}
Top & Bottom & Inputs& Acc & Pre& Rec& F1  \\
\midrule
\multirow{4}{*}{Swin-T \cite{liu2021swin}\footnotemark[1]} 
                                  & ResNet18 \cite{he2016deep}         & RGB+Shape & 80.62\%  & 78.68\%   & 74.93\% & 73.23\% \\ 
                                  & ResNet50 \cite{he2016deep}         & RGB+Shape & 80.45\%  & 75.44\%   & \textbf{76.21\%} & 72.68\% \\ 
                                  & Swin-T \cite{liu2021swin}\footnotemark[1] & RGB+Shape & 80.36\%         & \textbf{77.45\%}          & 75.81\%        & 73.33\%        \\ 
                                  & VGG19 \cite{simonyan2014very}            & RGB+Shape & \textbf{81.12\%}  & 76.28\%   & 75.73\% & \textbf{74.00\%} \\ 


% Validation Set  & 655  & 11.6\%  & 28(0.5\%)  & 69(1.2\%)  & 312(5.5\%)    & 246(4.4\%)\\
% Test Set        & 1,146& 20.2\%  & 48(0.8\%)  & 115(2.0\%) & 526(9.3\%)    & 457(8.1\%)\\
% Total           & 5,666& 100\%   & 222(3.9\%) & 612(10.8\%)& 2,540(44.8\%) & 2,292(40.5\%)\\
\botrule
\end{tabular*}
\footnotetext[1]{Swin-Transformer (Swin-T)}

\end{minipage}
\end{center}
\end{table}

% \begin{figure}[h!t]
%     \centering
%     \subfigure{
%         \includegraphics[width=2.5in]{Images/acc.png}
%         \includegraphics[width=2.5in]{Images/loss (1).png}
%     }
%     % \subfigure{
	
%     % }
    
%     \caption{Loss and accuracy curves for different models combined with SA module. The performance of Swin-Transformer\cite{liu2021swin} outperforms other models in terms of classification accuracy and classification loss.

%     }
%     \label{fig_6}
% \end{figure}

% \begin{figure}[h!t]
%     \centering
%     \includegraphics[scale=1.3]{Images/hybrid.png}
%     \caption{ Fluctuations in prediction classification accuracy of different network models with and without SA module. For clarity of presentation, we use abbreviations to denote the different network models (SA: Shape Attention, R18: ResNet18, R50: ResNet50, D121: DenseNet121, RN: ResNest, ST: Swin-Transformer).
%     }
%     \label{fig_7}
% \end{figure}

% \begin{figure*}[h!t]
%     \centering
%     \subfigure{
%         \includegraphics[width=2.5in]{Images/box_res18.png}
%         \includegraphics[width=2.5in]{Images/box_res50 (1).png}
%     }

%     \subfigure{
% 	\includegraphics[width=2.5in]{Images/densenet (1).png}
% 	\includegraphics[width=2.5in]{Images/resnest.png}
%     }
%     \subfigure{
% 	\includegraphics[width=2.5in]{Images/box_Swin_Transformer.png}
%     }
    
%     \caption{Fluctuation of model predictions with and without SA module.}
%     \label{fig.1}
% \end{figure*}
% This section will discuss the implementation details of our approach and the results of cell classification.

In this section, we first provide the implementation details of our method.
Then, we qualitatively evaluate the performance of different backbones in our dual-branch network and show the combination of Swin-Transformer (for RGB image) and VGG19 (for shape mask) can work best on our fine-grained BMEC dataset.
To further verify the effectiveness and generalizability of our shape-aware network, we compare the results on two WBC datasets and show our method can consistently achieve the best accuracy on different datasets.
In the end, we perform an ablation study to show the contribution of the shape attention module for improving the classification accuracy.
The code and BMEC dataset can be found on \url{https://github.com/wangye8899/BMEC}.

\subsection{Implementation Details}

The network architecture in Figure \ref{fig:overview} is implemented with the Timm \cite{rw2019timm} and PyTorch \cite{paszke2017automatic}. Both branch networks (Swin-Transformer, VGG19) are initialized with ImageNet pre-trained weights.
Furthermore, the shape attention module and cell classification network are initialized with Kaiming initialization \cite{KaimingHe2015DelvingDI}.
We adopt the SGD optimizer with a momentum of 0.9, weight decay of 2e-5
and a cosine lr schedule with the warm-up strategy \cite{loshchilov2016sgdr}. 
We set the warm-up learning rate to 1e-4, the maximum lr to 1e-3, and the minimum lr to 1e-4. 
Four data augmentation techniques are used: random crop, random horizontal flip with probability of 0.5, random vertical flip with probability of 0.5, and color jitter with factor of 0.4.
The network is trained for 300 epochs with batch size of 32 on three NVIDIA GTX 3090 GPUs and the total training takes 3 hours. 


\subsection{Classification Results on BMEC}
% \textcolor{raw}{We design a novel classification scheme based on Swin-Transformer\cite{liu2021swin} and shape attention module as shown in Figure \ref{fig:overview}. 
% For a comprehensive evaluation of our approach, we set up a total of four evaluation metrics, namely Accuracy, Precision, Recall, and F1-Score.
% Our method based on Swin-Transformer and shape attention achieves \textbf{81.12\%} Accuracy, \textbf{76.28\%} Precision, \textbf{75.73\%} Recall, and \textbf{74.00\%} F1-Score as shown in Table \ref{tab:backbone_top}, \ref{tab:backbone_bottom}.
% This demonstrates that our method possesses excellent performance and robustness.
% }
Our dual-branch network allows flexible choices of different backbone models for the cell classification.
To quantitatively evaluate the performance of different backbones for the two branches, we conducted classification experiments with various classic and SOTA image feature extraction models on our BMEC dataset and compared the results in Table \ref{tab:backbone_top} and \ref{tab:backbone_bottom}.
Since the RGB image in the top branch contains more color variations than the binary shape mask in the bottom branch, it is expected that a more complex backbone model is needed for the top branch, while a relative simple model may be sufficient for the bottom branch.
Therefore, in Table \ref{tab:backbone_top}, we fixed the bottom branch with a VGG19 which is a classic CNN based model and tested different backbones for the top branch.
It is shown the SOTA Swin-Transformer model can produce the best accuracy and F1 score comparing to other models such as ResNet \cite{he2016deep}, DenseNet \cite{huang2017densely} or ResNest \cite{HangZhang2020ResNeStSN} for extracting features from the RGB images.
Similarly, we fixed the top branch network as Swin-Transformer and evaluated different models for the bottom branch.
The results in Table \ref{tab:backbone_bottom} shows the VGG19 model is most suitable for the bottom branch, while one possible reason is that other models may underfit or overfit the binary shape mask images.
Based on above experiments, we finally choose Swin-Transformer and VGG19 for the top and bottom branches, and our final model achieved 81.12\% accuracy on BMEC.
Note that the backbones can always be easily evaluated and replaced when newer and more powerful image models are proposed.
% We have conducted numerous experiments to demonstrate the performance of our method, as shown in Table 4.


% \begin{table*}[h!t]
% \centering
% \begin{tabular}{|c|c|c|c|}
% \hline
% Study                          & Method                             & Category Number & Accuracy \\ \hline

% Kouzeh  et al. (2021) \cite{kouzehkanan2021raabin}            & VGG16        & 6              & 98.09\%  \\ \hline
% Kouzeh et al. (2021) \cite{kouzehkanan2021raabin}            & MnasNet1        & 6              & 98.59\%  \\ \hline

% Kouzeh et al. (2021) \cite{kouzehkanan2021raabin}            & DenseNet121        & 6              & 98.87\%  \\ \hline
% Kouzeh et al. (2021) \cite{kouzehkanan2021raabin}            & ShuffleNet-V2        & 6              & 99.03\%  \\ \hline
% Tavakoli et al. (2021) \cite{tavakoli2021new}            & Segmentation        & 6              & 94.65\%  \\ \hline
% % Muhammad Attique Khan al et. (2021) \cite{khan2021automated}            & Feature selection and ELM        & 4              & 96.60\%  \\ \hline

% Ours                     & Dual-Branch and Shape Attention & 6               & \textbf{99.17\%}    \\ \hline
% \end{tabular}
% \caption{Comparison of different methods for classification on Raabin-WBC dataset \cite{kouzehkanan2021raabin}.}
% \label{tab:rabbin}
% \end{table*}



\begin{table}[h]
\begin{center}
\begin{minipage}{\textwidth}
\caption{Ablation study on the shape information using our BMEC dataset.}\label{tab:ablation}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccc@{\extracolsep{\fill}}}
\toprule%
% & \multicolumn{6}{@{}c@{}}{BMEC Dataset Statistic} 
% \\\cmidrule{2-7}
Top & Bottom & Inputs& Acc & Pre& Rec& F1  \\
\midrule
\multirow{2}{*}{ResNet18 \cite{he2016deep}}         & ---                 & RGB       & 78.79\% & 71.91\% & 73.09\%&
                                  71.77\%
\\ 
                                  & VGG19 \cite{simonyan2014very}               & RGB+Shape & 79.51\% & 74.27\%&
                                  73.54\%& 72.42\%    \\
                                  \hline
                                  
\multirow{2}{*}{ResNet50 \cite{he2016deep}}         & ---                 & RGB       & 79.31\%   & 72.16\%          
                                  & 73.18\%   & 71.85\%    \\ 
                                  & VGG19 \cite{simonyan2014very}               & RGB+Shape & 79.58\%    & 74.33\%          
                                  & 73.67\% & 72.51\%   \\ \hline
                                  
\multirow{2}{*}{DenseNet121 \cite{huang2017densely}}      & ---                 & RGB       & 79.30\%    & 71.45\%           
                                  & 72.23\%     & 70.91\%     \\ 
                                  & VGG19 \cite{simonyan2014very}               & RGB+Shape & 79.65\%   & 73.42\%
                                  & 73.15\% & 72.20\%    \\ \hline
                                  
\multirow{2}{*}{ResNest \cite{HangZhang2020ResNeStSN}}          & ---           & RGB       & 80.09\%    & 74.49\%          
                                  & 73.95\%      &72.87\%    \\ 
                                  & VGG19 \cite{simonyan2014very}               & RGB+Shape & 80.12\%    & \textbf{76.47\%}
                                  & 74.64\% & 73.04\%   \\ \hline
                                  
\multirow{2}{*}{Swin-T \cite{liu2021swin}\footnotemark[1]} & ---                 & RGB       & 80.62\%    & 75.81\%                                         &74.79\%     & 72.85\%    \\  
                                  & VGG19 \cite{simonyan2014very}               & RGB+Shape & \textbf{81.12\%}    & 76.28\%
                                  &\textbf{75.73\%} & \textbf{74.00\%}    \\ 
                                  


% Validation Set  & 655  & 11.6\%  & 28(0.5\%)  & 69(1.2\%)  & 312(5.5\%)    & 246(4.4\%)\\
% Test Set        & 1,146& 20.2\%  & 48(0.8\%)  & 115(2.0\%) & 526(9.3\%)    & 457(8.1\%)\\
% Total           & 5,666& 100\%   & 222(3.9\%) & 612(10.8\%)& 2,540(44.8\%) & 2,292(40.5\%)\\
\botrule
\end{tabular*}
% \footnotetext[1]{RGB image+Shape Mask image (RGB+S)}
\footnotetext[1]{Swin-Transformer (Swin-T)}

\end{minipage}
\end{center}
\end{table}


% \begin{table*}[htbp]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% Top branch network               & Bottom branch network & Inputs    & Accuracy     & Precision & Recall & F1 \\ \hline
% \multirow{2}{*}{ResNet18 \cite{he2016deep}}         & ---                 & RGB       & 78.79\% & 71.91\% & 73.09\%&
%                                   71.77\%
% \\ \cline{2-7} 
%                                   & VGG19 \cite{simonyan2014very}               & RGB+Shape & 79.51\% & 74.27\%&
%                                   73.54\%& 72.42\%    \\ \hline
                                  
% \multirow{2}{*}{ResNet50 \cite{he2016deep}}         & ---                 & RGB       & 79.31\%   & 72.16\%          
%                                   & 73.18\%   & 71.85\%    \\ \cline{2-7} 
%                                   & VGG19 \cite{simonyan2014very}               & RGB+Shape & 79.58\%    & 74.33\%          
%                                   & 73.67\% & 72.51\%   \\ \hline
                                  
% \multirow{2}{*}{DenseNet121 \cite{huang2017densely}}      & ---                 & RGB       & 79.30\%    & 71.45\%           
%                                   & 72.23\%     & 70.91\%     \\ \cline{2-7} 
%                                   & VGG19 \cite{simonyan2014very}               & RGB+Shape & 79.65\%   & 73.42\%
%                                   & 73.15\% & 72.20\%    \\ \hline
                                  
% \multirow{2}{*}{ResNest \cite{HangZhang2020ResNeStSN}}          & ---           & RGB       & 80.09\%    & 74.49\%          
%                                   & 73.95\%      &72.87\%    \\ \cline{2-7} 
%                                   & VGG19 \cite{simonyan2014very}               & RGB+Shape & 80.12\%    & \textbf{76.47\%}
%                                   & 74.64\% & 73.04\%   \\ \hline
                                  
% \multirow{2}{*}{Swin-Transformer \cite{liu2021swin}} & ---                 & RGB       & 80.62\%    & 75.81\%                                         &74.79\%     & 72.85\%    \\ \cline{2-7} 
%                                   & VGG19 \cite{simonyan2014very}               & RGB+Shape & \textbf{81.12\%}    & 76.28\%
%                                   &\textbf{75.73\%} & \textbf{74.00\%}    \\ \hline
% \end{tabular}
% \caption{Ablation study on the shape information using our BMEC dataset.
% % For each model and each set of inputs, we take the average result of 5 experiments as the final accuracy to eliminate the experimental fluctuations.
% % \textcolor{wy}{When the input is RGB image , we just employ the top branch network to complete the classification directly.
% % When the input is RGB image and Shape mask image, we utilize the two-branch network and combine it with the shape attention module to complete the classification.}
% }
% \label{tab:ablation}
% \end{table*}


\subsection{Classification Results on WBCs Datasets}

\begin{table}[h]
\begin{center}
\begin{minipage}{\textwidth}
\caption{Comparison of different methods for classification on LISC dataset \cite{rezatofighi2011automatic}. Due to the data imbalance problem in LISC, other methods directly discarded the cell categories with a low number of images. In contrast, we trained and tested using all categories and still obtained the best accuracy.}\label{tab:lisc}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccc@{\extracolsep{\fill}}}
\toprule%
% & \multicolumn{6}{@{}c@{}}{BMEC Dataset Statistic} 
% \\\cmidrule{2-7}
Study& Method& Category Number & Accuracy  \\
\midrule
Rezatofighi et al. (2011) \cite{rezatofighi2011automatic} & SVM                               & 5               & 96.00\%  \\ 
Jung et al. (2019) \cite{jung2019w}                      & CNN                   & 5               & 97.00\%  \\

Baydilli et al. (2020) \cite{baydilli2020classification}              & Capsule Networks        & 5               & 96.86\%  \\ 
Harshanand et al. (2020)  \cite{harshanand2020comprehensive}              & CNN         & 5               & 97.64\%  \\ 
Tavakoli et al. (2021) \cite{tavakoli2021new}                        & Segmentation                      & 5               & 92.21\%  \\ 
Muhammad et al. (2021) \cite{khan2021automated}            & Feature Selection and ELM        & 4              & 96.60\%  \\ 

Ours                      & DB and SA\footnotemark[1] & 6              & \textbf{98.51\%}    \\ 

% Validation Set  & 655  & 11.6\%  & 28(0.5\%)  & 69(1.2\%)  & 312(5.5\%)    & 246(4.4\%)\\
% Test Set        & 1,146& 20.2\%  & 48(0.8\%)  & 115(2.0\%) & 526(9.3\%)    & 457(8.1\%)\\
% Total           & 5,666& 100\%   & 222(3.9\%) & 612(10.8\%)& 2,540(44.8\%) & 2,292(40.5\%)\\
\botrule
\end{tabular*}
\footnotetext[1]{Dual Branch and Shape Attention (DB and SA)}

\end{minipage}
\end{center}
\end{table}

\begin{table}[h]
\begin{center}
\begin{minipage}{\textwidth}
\caption{Comparison of different methods for classification on Raabin-WBC dataset \cite{kouzehkanan2021raabin}.}\label{tab:rabbin}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccc@{\extracolsep{\fill}}}
\toprule%
% & \multicolumn{6}{@{}c@{}}{BMEC Dataset Statistic} 
% \\\cmidrule{2-7}
Study& Method& Category Number & Accuracy \\ 
\midrule
Kouzeh  et al. (2021) \cite{kouzehkanan2021raabin}            & VGG16        & 6              & 98.09\%  \\ 
Kouzeh et al. (2021) \cite{kouzehkanan2021raabin}            & MnasNet1        & 6              & 98.59\%  \\ 

Kouzeh et al. (2021) \cite{kouzehkanan2021raabin}            & DenseNet121        & 6              & 98.87\%  \\ 
Kouzeh et al. (2021) \cite{kouzehkanan2021raabin}            & ShuffleNet-V2        & 6              & 99.03\%  \\
Tavakoli et al. (2021) \cite{tavakoli2021new}            & Segmentation        & 6              & 94.65\%  \\ 
% Muhammad Attique Khan al et. (2021) \cite{khan2021automated}            & Feature selection and ELM        & 4              & 96.60\%  \\ \hline

Ours                     & DB and SA\footnotemark[1] & 6               & \textbf{99.17\%}    \\ 

% Validation Set  & 655  & 11.6\%  & 28(0.5\%)  & 69(1.2\%)  & 312(5.5\%)    & 246(4.4\%)\\
% Test Set        & 1,146& 20.2\%  & 48(0.8\%)  & 115(2.0\%) & 526(9.3\%)    & 457(8.1\%)\\
% Total           & 5,666& 100\%   & 222(3.9\%) & 612(10.8\%)& 2,540(44.8\%) & 2,292(40.5\%)\\
\botrule
\end{tabular*}
\footnotetext[1]{Dual Branch and Shape Attention (DB and SA)}

\end{minipage}
\end{center}
\end{table}



\textcolor{raw}{To further demonstrate the effectiveness of our shape-aware network, we conducted classification experiments on two other public WBCs datasets, LISC \cite{rezatofighi2011automatic} and Raabin-WBC \cite{kouzehkanan2021raabin}.
We retrained our model using their training data and compared the testing results with the reported numbers in \cite{rezatofighi2011automatic} and \cite{kouzehkanan2021raabin}.
As shown in Table \ref{tab:lisc} and \ref{tab:rabbin}}, we achieved the best classification accuracy on both datasets, showing the generalizability of our method.
In addition, the high accuracy (over 98.5\%) on both WBC datasets indicates the classification of WBCs is relatively easier than the erythroid cells since the shape differences of WBCs are more prominent.
We hope our BMEC dataset can inspire and facilitate more research on fine-grained classification and other learning tasks for erythroid cells. 

\subsection{Ablation Study on Shape information}
\label{sec:ablation}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% \textbf{\textcolor{wy}{The Effectiveness of SA module}}:
% \textcolor{wy}{
% To demonstrate the validity of our SA module, we have applied the SA module to several models, including ResNet18\cite{he2016deep}, ResNet50\cite{he2016deep}, DenseNet121\cite{huang2017densely}, ResNest\cite{HangZhang2020ResNeStSN}, and Swin-Transformer\cite{liu2021swin}.
% As shown in Table \ref{table_9}, 
% on the above five models, the accuracy, precision, recall, and F1 are improved on average by \textbf{0.37\%}, \textbf{1.93\%}, \textbf{0.70\%}, and \textbf{0.78\%}, respectively, when using the SA module. 
% Regardless of which model is used, the average metrics are improved when utilizing the SA module to highlight shape features for classification.
% This indicates that the SA module, a simple but effective component, can efficiently highlight and fuse shape information to improve the classification results.
% }

To verify the effectiveness of the shape information, we performed an ablation study which compared our full dual-branch network with the RGB-only single branch network (see Table \ref{tab:ablation}).
Specifically, we disabled the bottom branch and only used the raw image feature for classification.
In this case, the network becomes a conventional RGB image based classification model.
When two branches are enabled, both the shape feature extracted from the binary shape mask and shape-attended image feature computed from the shape attention module are fused to the raw image feature for classification.
For the single branch network, different backbone models are tested on the BMEC RGB images.
For our dual-branch network, the VGG19 is used in each configuration so that we can compare the performance improvement for each case.
From the results in Table \ref{tab:ablation}, the dual-branch network can always outperform the single-branch, confirming the effectiveness of the shape information for improving the fine-grained cell classification.





% \textbf{\textcolor{review}{Training stability of SA module}}:
% As shown in Figure \ref{fig_6}, we use box plots to represent the volatility of the model predictions.
% When the SA module is applied, the classification results are improved, and the training and inference of the model are more stable.
% This demonstrates that the shape information highlighted by the SA module can make model training and prediction more steady.  


% \textbf{\textcolor{wy}{Top branch network}}:
% \textcolor{wy}{
% To discover the optimal top branch network selection, we first fix the down branch network as VGG19 and then try different backbone networks as the top branch network in our classification scheme. As shown in Table \ref{tab:backbone_top}, the best accuracy (\textbf{81.12\%}), recall (\textbf{75.73\%}) and F1-Score (\textbf{74.00\%}) are achieved when Swin-Transformer is utilized as the top branch network. 
% As shown in Figure \ref{fig_6},
% Swin-Transformer achieved lower training loss and higher classification performance than other models. 
% This indicates that Swin-Transformer can extract significant information and features from the complex RGB cell images. 
% Therefore, we adopt Swin-Transformer as the top branch network of our method.
% }


% \textbf{\textcolor{wy}{Down branch network:}}
% \textcolor{wy}{
% After determining the optimal top branch network as Swin-Transformer, we try different network models (VGG19, ResNet18, ResNet50, Swin-Transformer) as the down branch network.
% As shown in Table \ref{tab:backbone_bottom}, the best accuracy (\textbf{81.12\%}) and F1-Score (\textbf{74.00\%}) are achieved when the down branch network is selected as VGG19. 
% We concluded that VGG19 is optimal as the down branch network through comprehensive analysis.
% After extensive experiments and analysis, we finally adopt the combination of Swin-Transformer as the top branch network and VGG19 as the down branch network.
% }








==> 06Conclusion.tex <==
\section{Conclusion, Limitation and Future Work}
% We introduce the most extensive dataset on erythroid cell images for the first time.
% This dataset contains 5,666 images of four types of erythroid cells: proerythroblast, basophilic erythroblast, polychromatophilic erythroblast, and orthochromic erythrobla. 
% We design a simple but effective component called the Shape Attention module, which can be flexibly applied to other backbone networks. It can efficiently utilize the shape information to improve the classification results.
% We propose a new classification scheme based on the Swin-Transformer and combined with the SA module. Experimental results on several datasets demonstrate the effectiveness of our approach.
% In the future, we plan to design a more efficient feature fusion method based on attention techniques.
% Besides, We plan to propose a more lightweight network model by improving the Swin-Transformer.

We introduce BMEC, the first and largest professionally annotated image dataset for fine-grained classification of erythroid cells.
The BMEC is public available for all communities and we hope it can encourage more deep learning research on erythroid cells.
We propose a novel shape-aware network which explicitly utilizes the shape information to improve the classification accuracy in a dual-branch deep learning framework.
Extensive evaluations of different backbones, experiments on different datasets, as well as an ablation study are conducted and the results verify the effectiveness of our method.

Although our method has achieved superior performance on cell classification, it still has some limitations which can inspire more future work.
Our current cell shape extraction still involves several image processing steps which may be affected by the image noise and staining quality.
It will be interesting to automatically learn the cell shape segmentation in the network and then apply the learned shape mask in our dual-branch network.
Meanwhile, our classification works on the cropped cell images which are prepared in the BMEC dataset.
Developing a cell detection and classification network which can directly work on the full-field cell images is also a promising future work.
Due to the privacy issue, we cannot release the full-field cell images used in our BMEC, but it is still possible to train a cell detection network using the cropped BMEC cell images.


==> 07declarations.tex <==
\section*{Declarations}


\begin{itemize}
\item Funding: This research is supported by the National Natural Science Foundation of China (Grants No. 61772227, 61972174, 61972175), 
Science and Technology Development Foundation of Jilin Province (No. 20180201045GX, 20200201300JC, 20200401083GX, 20200201163JC), 
the Jilin Development and Reform Commission Fund (No. 2020C020-2).
\item Conflict of interest/Competing interests: The authors declare no conflict of interest.
\item Availability of data and materials: The code and dataset have been published on github (\url{https://github.com/wangye8899/BMEC}).
\item Code availability: \url{https://github.com/wangye8899/BMEC}
\item Authors' contributions: Conceptualization, Y.W. and R.M.; methodology, Y.W., R.M. and Y.Z.; validation, X.M., Y.X. and X.W.; formal analysis, Y.W. and R.M.; investigation, H.C.; resources, Y.Z.; data curation, H.C. and X.M.; writing---original draft preparation, Y.W.; writing---review and editing, R.M.; visualization, Y.W. and R.M.; supervision, Y.Z.; project administration, Y.Z.; All authors have read and agreed to the published version of the manuscript.
\end{itemize}

% \noindent
% If any of the sections are not relevant to your manuscript, please include the heading and write `Not applicable' for that section. 

% %%===================================================%%
% %% For presentation purpose, we have included        %%
% %% \bigskip command. please ignore this.             %%
% %%===================================================%%
% \bigskip
% \begin{flushleft}%
% Editorial Policies for:

% \bigskip\noindent
% Springer journals and proceedings: \url{https://www.springer.com/gp/editorial-policies}

% \bigskip\noindent
% Nature Portfolio journals: \url{https://www.nature.com/nature-research/editorial-policies}

% \bigskip\noindent
% \textit{Scientific Reports}: \url{https://www.nature.com/srep/journal-policies/editorial-policies}

% \bigskip\noindent
% BMC journals: \url{https://www.biomedcentral.com/getpublished/editorial-policies}
% \end{flushleft}

% \begin{appendices}


==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}



==> style.tex <==
\section{Results}\label{sec2}

Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

\section{This is an example for first level head---section head}\label{sec3}

\subsection{This is an example for second level head---subsection head}\label{subsec2}

\subsubsection{This is an example for third level head---subsubsection head}\label{subsubsec2}

Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. 

\section{Equations}\label{sec4}

Equations in \LaTeX\ can either be inline or on-a-line by itself (``display equations''). For
inline equations use the \verb+$...$+ commands. E.g.: The equation
$H\psi = E \psi$ is written via the command \verb+$H \psi = E \psi$+.

For display equations (with auto generated equation numbers)
one can use the equation or align environments:
\begin{equation}
\|\tilde{X}(k)\|^2 \leq\frac{\sum\limits_{i=1}^{p}\left\|\tilde{Y}_i(k)\right\|^2+\sum\limits_{j=1}^{q}\left\|\tilde{Z}_j(k)\right\|^2 }{p+q}.\label{eq1}
\end{equation}
where,
\begin{align}
D_\mu &=  \partial_\mu - ig \frac{\lambda^a}{2} A^a_\mu \nonumber \\
F^a_{\mu\nu} &= \partial_\mu A^a_\nu - \partial_\nu A^a_\mu + g f^{abc} A^b_\mu A^a_\nu \label{eq2}
\end{align}
Notice the use of \verb+\nonumber+ in the align environment at the end
of each line, except the last, so as not to produce equation numbers on
lines where no equation numbers are required. The \verb+\label{}+ command
should only be used at the last line of an align environment where
\verb+\nonumber+ is not used.
\begin{equation}
Y_\infty = \left( \frac{m}{\textrm{GeV}} \right)^{-3}
    \left[ 1 + \frac{3 \ln(m/\textrm{GeV})}{15}
    + \frac{\ln(c_2/5)}{15} \right]
\end{equation}
The class file also supports the use of \verb+\mathbb{}+, \verb+\mathscr{}+ and
\verb+\mathcal{}+ commands. As such \verb+\mathbb{R}+, \verb+\mathscr{R}+
and \verb+\mathcal{R}+ produces $\mathbb{R}$, $\mathscr{R}$ and $\mathcal{R}$
respectively (refer Subsubsection~\ref{subsubsec2}).

\section{Tables}\label{sec5}

Tables can be inserted via the normal table and tabular environment. To put
footnotes inside tables you should use \verb+\footnotetext[]{...}+ tag.
The footnote appears just below the table itself (refer Tables~\ref{tab1} and \ref{tab2}). 
For the corresponding footnotemark use \verb+\footnotemark[...]+

\begin{table}[h]
\begin{center}
\begin{minipage}{174pt}
\caption{Caption text}\label{tab1}%
\begin{tabular}{@{}llll@{}}
\toprule
Column 1 & Column 2  & Column 3 & Column 4\\
\midrule
row 1    & data 1   & data 2  & data 3  \\
row 2    & data 4   & data 5\footnotemark[1]  & data 6  \\
row 3    & data 7   & data 8  & data 9\footnotemark[2]  \\
\botrule
\end{tabular}
\footnotetext{Source: This is an example of table footnote. This is an example of table footnote.}
\footnotetext[1]{Example for a first table footnote. This is an example of table footnote.}
\footnotetext[2]{Example for a second table footnote. This is an example of table footnote.}
\end{minipage}
\end{center}
\end{table}

\noindent
The input format for the above table is as follows:

%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. please ignore this.       %%
%%=============================================%%
\bigskip
\begin{verbatim}
\begin{table}[<placement-specifier>]
\begin{center}
\begin{minipage}{<preferred-table-width>}
\caption{<table-caption>}\label{<table-label>}%
\begin{tabular}{@{}llll@{}}
\toprule
Column 1 & Column 2 & Column 3 & Column 4\\
\midrule
row 1 & data 1 & data 2	 & data 3 \\
row 2 & data 4 & data 5\footnotemark[1] & data 6 \\
row 3 & data 7 & data 8	 & data 9\footnotemark[2]\\
\botrule
\end{tabular}
\footnotetext{Source: This is an example of table footnote. 
This is an example of table footnote.}
\footnotetext[1]{Example for a first table footnote.
This is an example of table footnote.}
\footnotetext[2]{Example for a second table footnote. 
This is an example of table footnote.}
\end{minipage}
\end{center}
\end{table}
\end{verbatim}
\bigskip
%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. please ignore this.       %%
%%=============================================%%

\begin{table}[h]
\begin{center}
\begin{minipage}{\textwidth}
\caption{Example of a lengthy table which is set to full textwidth}\label{tab2}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccc@{\extracolsep{\fill}}}
\toprule%
& \multicolumn{3}{@{}c@{}}{Element 1\footnotemark[1]} & \multicolumn{3}{@{}c@{}}{Element 2\footnotemark[2]} \\\cmidrule{2-4}\cmidrule{5-7}%
Project & Energy & $\sigma_{calc}$ & $\sigma_{expt}$ & Energy & $\sigma_{calc}$ & $\sigma_{expt}$ \\
\midrule
Element 3  & 990 A & 1168 & $1547\pm12$ & 780 A & 1166 & $1239\pm100$\\
Element 4  & 500 A & 961  & $922\pm10$  & 900 A & 1268 & $1092\pm40$\\
\botrule
\end{tabular*}
\footnotetext{Note: This is an example of table footnote. This is an example of table footnote this is an example of table footnote this is an example of~table footnote this is an example of table footnote.}
\footnotetext[1]{Example for a first table footnote.}
\footnotetext[2]{Example for a second table footnote.}
\end{minipage}
\end{center}
\end{table}

In case of double column layout, tables which do not fit in single column width should be set to full text width. For this, you need to use \verb+\begin{table*}+ \verb+...+ \verb+\end{table*}+ instead of \verb+\begin{table}+ \verb+...+ \verb+\end{table}+ environment. Lengthy tables which do not fit in textwidth should be set as rotated table. For this, you need to use \verb+\begin{sidewaystable}+ \verb+...+ \verb+\end{sidewaystable}+ instead of \verb+\begin{table*}+ \verb+...+ \verb+\end{table*}+ environment. This environment puts tables rotated to single column width. For tables rotated to double column width, use \verb+\begin{sidewaystable*}+ \verb+...+ \verb+\end{sidewaystable*}+.

\begin{sidewaystable}
\sidewaystablefn%
\begin{center}
\begin{minipage}{\textheight}
\caption{Tables which are too long to fit, should be written using the ``sidewaystable'' environment as shown here}\label{tab3}
\begin{tabular*}{\textheight}{@{\extracolsep{\fill}}lcccccc@{\extracolsep{\fill}}}
\toprule%
& \multicolumn{3}{@{}c@{}}{Element 1\footnotemark[1]}& \multicolumn{3}{@{}c@{}}{Element\footnotemark[2]} \\\cmidrule{2-4}\cmidrule{5-7}%
Projectile & Energy	& $\sigma_{calc}$ & $\sigma_{expt}$ & Energy & $\sigma_{calc}$ & $\sigma_{expt}$ \\
\midrule
Element 3 & 990 A & 1168 & $1547\pm12$ & 780 A & 1166 & $1239\pm100$ \\
Element 4 & 500 A & 961  & $922\pm10$  & 900 A & 1268 & $1092\pm40$ \\
Element 5 & 990 A & 1168 & $1547\pm12$ & 780 A & 1166 & $1239\pm100$ \\
Element 6 & 500 A & 961  & $922\pm10$  & 900 A & 1268 & $1092\pm40$ \\
\botrule
\end{tabular*}
\footnotetext{Note: This is an example of table footnote this is an example of table footnote this is an example of table footnote this is an example of~table footnote this is an example of table footnote.}
\footnotetext[1]{This is an example of table footnote.}
\end{minipage}
\end{center}
\end{sidewaystable}

\section{Figures}\label{sec6}

As per the \LaTeX\ standards you need to use eps images for \LaTeX\ compilation and \verb+pdf/jpg/png+ images for \verb+PDFLaTeX+ compilation. This is one of the major difference between \LaTeX\ and \verb+PDFLaTeX+. Each image should be from a single input .eps/vector image file. Avoid using subfigures. The command for inserting images for \LaTeX\ and \verb+PDFLaTeX+ can be generalized. The package used to insert images in \verb+LaTeX/PDFLaTeX+ is the graphicx package. Figures can be inserted via the normal figure environment as shown in the below example:

%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. please ignore this.       %%
%%=============================================%%
\bigskip
\begin{verbatim}
\begin{figure}[<placement-specifier>]
\centering
\includegraphics{<eps-file>}
\caption{<figure-caption>}\label{<figure-label>}
\end{figure}
\end{verbatim}
\bigskip
%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. please ignore this.       %%
%%=============================================%%

\begin{figure}[h]%
\centering
\includegraphics[width=0.9\textwidth]{fig.eps}
\caption{This is a widefig. This is an example of long caption this is an example of long caption  this is an example of long caption this is an example of long caption}\label{fig1}
\end{figure}

In case of double column layout, the above format puts figure captions/images to single column width. To get spanned images, we need to provide \verb+\begin{figure*}+ \verb+...+ \verb+\end{figure*}+.

For sample purpose, we have included the width of images in the optional argument of \verb+\includegraphics+ tag. Please ignore this. 

\section{Algorithms, Program codes and Listings}\label{sec7}

Packages \verb+algorithm+, \verb+algorithmicx+ and \verb+algpseudocode+ are used for setting algorithms in \LaTeX\ using the format:

%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. please ignore this.       %%
%%=============================================%%
\bigskip
\begin{verbatim}
\begin{algorithm}
\caption{<alg-caption>}\label{<alg-label>}
\begin{algorithmic}[1]
. . .
\end{algorithmic}
\end{algorithm}
\end{verbatim}
\bigskip
%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. please ignore this.       %%
%%=============================================%%

You may refer above listed package documentations for more details before setting \verb+algorithm+ environment. For program codes, the ``program'' package is required and the command to be used is \verb+\begin{program}+ \verb+...+ \verb+\end{program}+. A fast exponentiation procedure:

\begin{program}
\BEGIN \\ %
  \FOR i:=1 \TO 10 \STEP 1 \DO
     |expt|(2,i); \\ |newline|() \OD %
\rcomment{Comments will be set flush to the right margin}
\WHERE
\PROC |expt|(x,n) \BODY
          z:=1;
          \DO \IF n=0 \THEN \EXIT \FI;
             \DO \IF |odd|(n) \THEN \EXIT \FI;
\COMMENT{This is a comment statement};
                n:=n/2; x:=x*x \OD;
             \{ n>0 \};
             n:=n-1; z:=z*x \OD;
          |print|(z) \ENDPROC
\END
\end{program}


\begin{algorithm}
\caption{Calculate $y = x^n$}\label{algo1}
\begin{algorithmic}[1]
\Require $n \geq 0 \vee x \neq 0$
\Ensure $y = x^n$ 
\State $y \Leftarrow 1$
\State $a = 1$


\end{algorithmic}
\end{algorithm}
\bigskip
%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. please ignore this.       %%
%%=============================================%%

Similarly, for \verb+listings+, use the \verb+listings+ package. \verb+\begin{lstlisting}+ \verb+...+ \verb+\end{lstlisting}+ is used to set environments similar to \verb+verbatim+ environment. Refer to the \verb+lstlisting+ package documentation for more details.

%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. please ignore this.       %%
%%=============================================%%
\bigskip
\begin{minipage}{\hsize}%
\lstset{frame=single,framexleftmargin=-1pt,framexrightmargin=-17pt,framesep=12pt,linewidth=0.98\textwidth,language=pascal}% Set your language (you can change the language for each code-block optionally)
%%% Start your code-block
\begin{lstlisting}
for i:=maxint to 0 do
begin
{ do nothing }
end;
Write('Case insensitive ');
Write('Pascal keywords.');
\end{lstlisting}
\end{minipage}

\section{Cross referencing}\label{sec8}

Environments such as figure, table, equation and align can have a label
declared via the \verb+\label{#label}+ command. For figures and table
environments use the \verb+\label{}+ command inside or just
below the \verb+\caption{}+ command. You can then use the
\verb+\ref{#label}+ command to cross-reference them. As an example, consider
the label declared for Figure~\ref{fig1} which is
\verb+\label{fig1}+. To cross-reference it, use the command 
\verb+Figure \ref{fig1}+, for which it comes up as
``Figure~\ref{fig1}''. 

To reference line numbers in an algorithm, consider the label declared for the line number 2 of Algorithm~\ref{algo1} is \verb+\label{algln2}+. To cross-reference it, use the command \verb+\ref{algln2}+ for which it comes up as line~\ref{algln2} of Algorithm~\ref{algo1}.

\subsection{Details on reference citations}\label{subsec7}

Standard \LaTeX\ permits only numerical citations. To support both numerical and author-year citations this template uses \verb+natbib+ \LaTeX\ package. For style guidance please refer to the template user manual.

Here is an example for \verb+\cite{...}+: \cite{bib1}. Another example for \verb+\citep{...}+: \citep{bib2}. For author-year citation mode, \verb+\cite{...}+ prints Jones et al. (1990) and \verb+\citep{...}+ prints (Jones et al., 1990).

All cited bib entries are printed at the end of this article: \cite{bib3}, \cite{bib4}, \cite{bib5}, \cite{bib6}, \cite{bib7}, \cite{bib8}, \cite{bib9}, \cite{bib10}, \cite{bib11} and \cite{bib12}.

\section{Examples for theorem like environments}\label{sec10}

For theorem like environments, we require \verb+amsthm+ package. There are three types of predefined theorem styles exists---\verb+thmstyleone+, \verb+thmstyletwo+ and \verb+thmstylethree+ 

%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. please ignore this.       %%
%%=============================================%%
\bigskip
\begin{tabular}{|l|p{19pc}|}
\hline
\verb+thmstyleone+ & Numbered, theorem head in bold font and theorem text in italic style \\\hline
\verb+thmstyletwo+ & Numbered, theorem head in roman font and theorem text in italic style \\\hline
\verb+thmstylethree+ & Numbered, theorem head in bold font and theorem text in roman style \\\hline
\end{tabular}
\bigskip
%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. please ignore this.       %%
%%=============================================%%

For mathematics journals, theorem styles can be included as shown in the following examples:

\begin{theorem}[Theorem subhead]\label{thm1}
Example theorem text. Example theorem text. Example theorem text. Example theorem text. Example theorem text. 
Example theorem text. Example theorem text. Example theorem text. Example theorem text. Example theorem text. 
Example theorem text. 
\end{theorem}

Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

\begin{proposition}
Example proposition text. Example proposition text. Example proposition text. Example proposition text. Example proposition text. 
Example proposition text. Example proposition text. Example proposition text. Example proposition text. Example proposition text. 
\end{proposition}

Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

\begin{example}
Phasellus adipiscing semper elit. Proin fermentum massa
ac quam. Sed diam turpis, molestie vitae, placerat a, molestie nec, leo. Maecenas lacinia. Nam ipsum ligula, eleifend
at, accumsan nec, suscipit a, ipsum. Morbi blandit ligula feugiat magna. Nunc eleifend consequat lorem. 
\end{example}

Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

\begin{remark}
Phasellus adipiscing semper elit. Proin fermentum massa
ac quam. Sed diam turpis, molestie vitae, placerat a, molestie nec, leo. Maecenas lacinia. Nam ipsum ligula, eleifend
at, accumsan nec, suscipit a, ipsum. Morbi blandit ligula feugiat magna. Nunc eleifend consequat lorem. 
\end{remark}

Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

\begin{definition}[Definition sub head]
Example definition text. Example definition text. Example definition text. Example definition text. Example definition text. Example definition text. Example definition text. Example definition text. 
\end{definition}

Additionally a predefined ``proof'' environment is available: \verb+\begin{proof}+ \verb+...+ \verb+\end{proof}+. This prints a ``Proof'' head in italic font style and the ``body text'' in roman font style with an open square at the end of each proof environment. 

\begin{proof}
Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. 
\end{proof}

Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

\begin{proof}[Proof of Theorem~{\upshape\ref{thm1}}]
Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. 
\end{proof}

\noindent
For a quote environment, use \verb+\begin{quote}...\end{quote}+
\begin{quote}
Quoted text example. Aliquam porttitor quam a lacus. Praesent vel arcu ut tortor cursus volutpat. In vitae pede quis diam bibendum placerat. Fusce elementum
convallis neque. Sed dolor orci, scelerisque ac, dapibus nec, ultricies ut, mi. Duis nec dui quis leo sagittis commodo.
\end{quote}

Sample body text. Sample body text. Sample body text. Sample body text. Sample body text (refer Figure~\ref{fig1}). Sample body text. Sample body text. Sample body text (refer Table~\ref{tab3}). 

\section{Methods}\label{sec11}

Topical subheadings are allowed. Authors must ensure that their Methods section includes adequate experimental and characterization data necessary for others in the field to reproduce their work. Authors are encouraged to include RIIDs where appropriate. 

\textbf{Ethical approval declarations} (only required where applicable) Any article reporting experiment/s carried out on (i)~live vertebrate (or higher invertebrates), (ii)~humans or (iii)~human samples must include an unambiguous statement within the methods section that meets the following requirements: 

\begin{enumerate}[1.]
\item Approval: a statement which confirms that all experimental protocols were approved by a named institutional and/or licensing committee. Please identify the approving body in the methods section

\item Accordance: a statement explicitly saying that the methods were carried out in accordance with the relevant guidelines and regulations

\item Informed consent (for experiments involving humans or human tissue samples): include a statement confirming that informed consent was obtained from all participants and/or their legal guardian/s
\end{enumerate}

If your manuscript includes potentially identifying patient/participant information, or if it describes human transplantation research, or if it reports results of a clinical trial then  additional information will be required. Please visit (\url{https://www.nature.com/nature-research/editorial-policies}) for Nature Portfolio journals, (\url{https://www.springer.com/gp/authors-editors/journal-author/journal-author-helpdesk/publishing-ethics/14214}) for Springer Nature journals, or (\url{https://www.biomedcentral.com/getpublished/editorial-policies\#ethics+and+consent}) for BMC.

\section{Discussion}\label{sec12}

Discussions should be brief and focused. In some disciplines use of Discussion or `Conclusion' is interchangeable. It is not mandatory to use both. Some journals prefer a section `Results and Discussion' followed by a section `Conclusion'. Please refer to Journal-level guidance for any specific requirements. 

\section{Conclusion}\label{sec13}

Conclusions may be used to restate your hypothesis or research question, restate your major findings, explain the relevance and the added value of your work, highlight any limitations of your study, describe future directions for research and recommendations. 

In some disciplines use of Discussion or 'Conclusion' is interchangeable. It is not mandatory to use both. Please refer to Journal-level guidance for any specific requirements. 

\backmatter

\bmhead{Supplementary information}

If your article has accompanying supplementary file/s please state so here. 

Authors reporting data from electrophoretic gels and blots should supply the full unprocessed scans for key as part of their Supplementary information. This may be requested by the editorial team/s if it is missing.

Please refer to Journal-level guidance for any specific requirements.

\bmhead{Acknowledgments}

Acknowledgments are not compulsory. Where included they should be brief. Grant or contribution numbers may be acknowledged.

Please refer to Journal-level guidance for any specific requirements.

\section*{Declarations}

Some journals require declarations to be submitted in a standardised format. Please check the Instructions for Authors of the journal to which you are submitting to see if you need to complete this section. If yes, your manuscript must contain the following sections under the heading `Declarations':

\begin{itemize}
\item Funding
\item Conflict of interest/Competing interests (check journal-specific guidelines for which heading to use)
\item Ethics approval 
\item Consent to participate
\item Consent for publication
\item Availability of data and materials
\item Code availability 
\item Authors' contributions
\end{itemize}

\noindent
If any of the sections are not relevant to your manuscript, please include the heading and write `Not applicable' for that section. 

%%===================================================%%
%% For presentation purpose, we have included        %%
%% \bigskip command. please ignore this.             %%
%%===================================================%%
\bigskip
\begin{flushleft}%
Editorial Policies for:

\bigskip\noindent
Springer journals and proceedings: \url{https://www.springer.com/gp/editorial-policies}

\bigskip\noindent
Nature Portfolio journals: \url{https://www.nature.com/nature-research/editorial-policies}

\bigskip\noindent
\textit{Scientific Reports}: \url{https://www.nature.com/srep/journal-policies/editorial-policies}

\bigskip\noindent
BMC journals: \url{https://www.biomedcentral.com/getpublished/editorial-policies}
\end{flushleft}

\begin{appendices}

\section{Section title of first appendix}\label{secA1}

An appendix contains supplementary information that is not an essential part of the text itself but which may be helpful in providing a more comprehensive understanding of the research problem or it is information that is too cumbersome to be included in the body of the paper.

%%=============================================%%
%% For submissions to Nature Portfolio Journals %%
%% please use the heading ``Extended Data''.   %%
%%=============================================%%

%%=============================================================%%
%% Sample for another appendix section			       %%
%%=============================================================%%

%% \section{Example of another appendix section}\label{secA2}%
%% Appendices may be used for helpful, supporting or essential material that would otherwise 
%% clutter, break up or be distracting to the text. Appendices can consist of sections, figures, 
%% tables and equations etc.

\end{appendices}

